Projections of Model Spaces for Latent Graph Inference

Graph Neural Networks leverage the connectivity structure of graphs as an inductive bias. Latent graph inference focuses on learning an adequate graph structure to diffuse information on and improve the downstream performance of the model. In this work we employ stereographic projections of the hyperbolic and spherical model spaces, as well as products of Riemannian manifolds, for the purpose of latent graph inference. Stereographically projected model spaces achieve comparable performance to their non-projected counterparts, while providing theoretical guarantees that avoid divergence of the spaces when the curvature tends to zero. We perform experiments on both homophilic and heterophilic graphs.

==> tables/additional_number_of_layers.tex <==


\begin{table*}[htbp!]
    \centering
    \caption{Results for Physics and CS using two dDGM latent graph inference modules with a product manifold combining Euclidean, hyperbolic, and spherical model spaces.}
    
\scalebox{0.65}{
    \begin{tabular}{l clcc}
    \toprule 
         &
         &
         &
         \textbf{Physics} &  
         \textbf{CS} 
 
         
         \\ 
         \midrule
         
         Model & $k$ & \multicolumn{1}{c}{Layers} &
         \multicolumn{2}{c}{Accuracy $(\%)$ $\pm$ Standard Deviation}
         
         \\

         
         \midrule

         GCN-dDGM-EHS & 5&
         dDGM/GCN/GCN/GCN &
         $ \secondd{96.17 {\scriptstyle \pm 0.30}}$ &
         $ \first{92.06 {\scriptstyle \pm 0.83}}$  \\

         GCN-dDGM-EHS & 5&
         dDGM/GCN/dDGM/GCN/GCN &
         $ \first{96.18 {\scriptstyle \pm 0.31 }}$ &
         $ \thirdd{87.00 {\scriptstyle \pm 4.00}}$ \\

         % GCN-dDGM-EHS & 5&
         % dDGM/GCN/dDGM/GCN/dDGM/GCN &
         % $  {\scriptstyle \pm }$ &
         % $ {\scriptstyle \pm }$ &
         % $  {\scriptstyle \pm }$ \\ 
         
         \midrule

        
         GCN & N/A &
         GCN/GCN/GCN&
         $ \thirdd{95.51 {\scriptstyle \pm 0.34}}$&
         $ \secondd{87.28 {\scriptstyle \pm 1.54}}$ \\ 

         
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:additional_number_of_layers}
\end{table*}

==> tables/aero_summary_of_models.tex <==


\begin{table*}[htbp!]
    \centering
    \caption{Summary of model architectures for Aerothermodynamics.
    }
    
\scalebox{0.83}{
    \begin{tabular}{lc cccc}
    \toprule 
&  & &\multicolumn{3}{c}{Model}
    \\ \midrule
          &
& &
         \textbf{MLP} &  
         \textbf{GCN-dDGM}
         &  
         \textbf{GAT-dDGM}
         \\ \midrule

         
         
         No. Layer parameters & BatchNorm & Activation & \multicolumn{3}{c}{Layer type}
         \\\midrule
          & &  N/A & N/A & dDGM & dDGM
          \\\hdashline
         (No. features, 32) & No & ELU & Linear  & Graph Conv & Graph Attention
          \\ 
          (32, 16) & No & ELU & Linear  & Graph Conv & Graph Attention
          \\
          (16, 8) & No & ELU & Linear & Graph Conv & Graph Attention
          \\ 
          (8, 8) & Yes & ELU & Linear & Linear & Linear
          \\ 
          (8, 8) & Yes & ELU & Linear& Linear & Linear
          \\ 
          (8, No. classes) & No  & - & Linear  & Linear & Linear
          \\ 
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:Summary of model architecture aero}
\end{table*}

==> tables/aero_summary_table.tex <==
\begin{table*}[ht!]
    \centering
    \caption{Summary of properties for Aerothermodynamics dataset
    }
    
\scalebox{0.75}{
    \begin{tabular}{l cc}
    \toprule 
         &
         &
         \textbf{Aerothermodynamics}  
        
         \\ \midrule
         
         Homophily level &
         &
         N/A 
     
         
          \\ 
         
         Nodes &
        &
         1,456
   
          \\
          
        Features &
        & 1 
      
          \\
         
         Edges &
        &
        N/A 
    
          \\
         
         Classes &
        &
        4 
         \\
         
         Average Degree & 
        & N/A 
         
         
         \\

         Learning & 
        &
        Transductive 
         \\
         
         Task & 
        &
        Classification  
         \\
         Network Type & 
        & CFD simulation
  

         
         
         \\
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:aero_summary_table}
\end{table*}

==> tables/arxiv.tex <==



\begin{table*}[htbp!]
    \centering
    \caption{Results for OGB-Arxiv dataset using GATv2 diffusion layers and different latent graph inference modules.
    }
    
\scalebox{0.65}{
    \begin{tabular}{lc}
    \toprule 
         &
         \textbf{OGB-Arxiv}

         
          \\ 
         
         Nodes &
        
          169,343
          \\

    
         
         
          
        Features &
        
128
          
          \\

          Edges &

          1,166,243\\
         
         
         Classes &
        
         40 \\

         $k$
        &
         20 \\
        
         
        
         \midrule
         
         Model &
         \multicolumn{1}{c}{Accuracy $(\%)$ $\pm$ Standard Deviation}
         
         \\
          \midrule

        GATv2-dDGM$^{*}$-E &
         $ 64.34 {\scriptstyle \pm 0.40 }$\\

         GATv2-dDGM$^{*}$-H &
         $ 61.30 {\scriptstyle \pm 0.50}$\\

         GATv2-dDGM$^{*}$-S &
         $ 64.41 {\scriptstyle \pm 0.64 }$\\

         GATv2-dDGM$^{*}$-HH &
         $ 64.24 {\scriptstyle \pm 0.17}$\\

         GATv2-dDGM$^{*}$-SS &
         $ 64.05 {\scriptstyle \pm 0.29 }$\\

        GATv2-dDGM$^{*}$-EH &
         $ 64.08 {\scriptstyle \pm 1.01}$\\

         GATv2-dDGM$^{*}$-ES &
         $ 64.13 {\scriptstyle \pm 0.61}$\\

         GATv2-dDGM$^{*}$-HS &
         $ 64.45 {\scriptstyle \pm 0.12 }$\\

         GATv2-dDGM$^{*}$-EHS &
         $ \first{65.06 {\scriptstyle \pm 0.09 }}$\\

        \midrule

        GATv2-dDGM-E &
         $ \thirdd{64.65 {\scriptstyle \pm 0.01 }}$\\

         GATv2-dDGM-H &
         $ \secondd{65.05 {\scriptstyle \pm 0.10 }}$\\

         GATv2-dDGM-S &
         $ 64.60 {\scriptstyle \pm 0.16 }$\\

         GATv2-dDGM-HH &
         $ 64.00 {\scriptstyle \pm 0.36}$\\

         GATv2-dDGM-SS &
         $ 64.35 {\scriptstyle \pm 0.36}$\\

        GATv2-dDGM-EH &
         $ 64.00 {\scriptstyle \pm 0.76 }$\\

         GATv2-dDGM-ES &
         $ 64.37 {\scriptstyle \pm 0.04 }$\\

         GATv2-dDGM-HS &
         $ 61.00 {\scriptstyle \pm 1.12 }$\\

         GATv2-dDGM-EHS &
         $ 64.25 {\scriptstyle \pm 0.50 }$\\
         
         
         \midrule
         MLP$^{*}$ &
         $ 63.49 {\scriptstyle \pm 0.15 }$ \\ 

         GATv2 &
         $ 61.93 {\scriptstyle \pm 1.62}$ \\ 
         

         
         \bottomrule
         
        \end{tabular}}
    
    \label{tab:arxiv}
\end{table*}

==> tables/dgm_aero.tex <==


\begin{table*}[t!]
    \centering
    \caption{dDGM$^{*}$ and dDGM architectures for Aerothermodynamics.
    }
    
\scalebox{0.54}{
    \begin{tabular}{lcc cc}
    \toprule 
          & &
& 
         \textbf{dDGM$^{*}$} &  
         \textbf{dDGM}
         \\ \midrule

         
         
         No. Layer parameters & BatchNorm  & Activation & \multicolumn{2}{c}{Layer type}
         \\\hline
         ($\textrm{No. features}$, 32)  & No & ELU & Linear & Linear
          \\
          (32, 16 per model space)  & Yes (dDGM$^{*}$)/ No (dDGM) & ELU & Linear & Graph Conv 
          \\
          (16 per model space, 4 per model space) & Yes (dDGM$^{*}$)/ No (dDGM) & Sigmoid (dDGM$^{*}$)/ ELU (dDGM) & Linear & Graph Conv 
          \\
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:dDGM_aero}
\end{table*}

==> tables/dgm_arxiv.tex <==


\begin{table*}[htbp!]
    \centering
    \caption{dDGM$^{*}$ and dDGM architectures for OGB-Arxiv.
    }
    
\scalebox{0.74}{
    \begin{tabular}{lcc cc}
    \toprule 
          & &
& 
         \textbf{dDGM$^{*}$} &  
         \textbf{dDGM}
         \\ \midrule

         
         
         No. Layer parameters & BatchNorm  & Activation & \multicolumn{2}{c}{Layer type}
         \\\hline
         ($\textrm{No. features}$, 40)  & Yes & SiLU & Linear & Linear
          \\
          (40, 32 per model space)  & Yes (dDGM$^{*}$)/ No (dDGM) & SiLU & Linear & Graph Conv 
          \\
          (32 per model space, 16 per model space) & Yes (dDGM$^{*}$)/ No (dDGM) & SiLU & Linear & Graph Conv 
          \\
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:dDGM_arxiv}
\end{table*}

==> tables/dgm_brain.tex <==


\begin{table*}[t!]
    \centering
    \caption{dDGM$^{*}$ and dDGM architectures for TadPole.
    }
    
\scalebox{0.6}{
    \begin{tabular}{lcc cc}
    \toprule 
          & &
& 
         \textbf{dDGM$^{*}$} &  
         \textbf{dDGM}
         \\ \midrule

         
         
         No. Layer parameters & BatchNorm  & Activation & \multicolumn{2}{c}{Layer type}
         \\\hline
          ($\textrm{No. features}$, 16 per model space)  & Yes (dDGM$^{*}$)/ No (dDGM) & ELU & Linear & Graph Conv 
          \\
          (16 per model space, 4 per model space) & Yes (dDGM$^{*}$)/ No (dDGM) & Sigmoid (dDGM$^{*}$)/ ELU (dDGM) & Linear & Graph Conv 
          \\
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:dDGM_brain}
\end{table*}

==> tables/dgm_hetero.tex <==


\begin{table*}[htbp!]
    \centering
    \caption{dDGM$^{*}$ and dDGM architectures for heterophilic datasets.
    }
    
\scalebox{0.74}{
    \begin{tabular}{lcc cc}
    \toprule 
          & &
& 
         \textbf{dDGM$^{*}$} &  
         \textbf{dDGM}
         \\ \midrule

         
         
         No. Layer parameters & BatchNorm  & Activation & \multicolumn{2}{c}{Layer type}
         \\\hline
         ($\textrm{No. features}$, 32)  & Yes & ELU & Linear & Linear
          \\
          (32, 4 per model space)  & Yes (dDGM$^{*}$)/ No (dDGM) & ELU & Linear & Graph Conv 
          \\
          (4 per model space, 4 per model space) & Yes (dDGM$^{*}$)/ No (dDGM) & Sigmoid & Linear & Graph Conv 
          \\
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:dDGM_hetero}
\end{table*}

==> tables/dgm_homo.tex <==


\begin{table*}[htbp!]
    \centering
    \caption{dDGM$^{*}$ and dDGM architectures for classical homophilic datasets.
    }
    
\scalebox{1}{
    \begin{tabular}{lc cc}
    \toprule 
          &
& 
         \textbf{dDGM$^{*}$} &  
         \textbf{dDGM}
         \\ \midrule

         
         
         No. Layer parameters  & Activation & \multicolumn{2}{c}{Layer type}
         \\\hline
         ($\textrm{No. features}$, 32)  & ELU & Linear & Linear
          \\
          (32, 16 per model space)  & ELU & Linear & Graph Conv 
          \\
          (16 per model space, 4 per model space) & Sigmoid & Linear & Graph Conv 
          \\
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:dDGM_homo}
\end{table*}

==> tables/dgm_inductive.tex <==


\begin{table*}[htbp!]
    \centering
    \caption{dDGM$^{*}$ and dDGM architectures for QM9 and Alchemy.
    }
    
\scalebox{0.74}{
    \begin{tabular}{lcc cc}
    \toprule 
          & &
& 
         \textbf{dDGM$^{*}$} &  
         \textbf{dDGM}
         \\ \midrule

         
         
         No. Layer parameters & BatchNorm  & Activation & \multicolumn{2}{c}{Layer type}
         \\\hline
          ($\textrm{No. features}$, 3 per model space)  & Yes & SiLU & Linear & Graph Conv 
          \\
          (3 per model space, 3 per model space) & Yes & SiLU & Linear & Graph Conv 
          \\
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:dDGM_inductive}
\end{table*}

==> tables/dgm_products.tex <==


\begin{table*}[htbp!]
    \centering
    \caption{dDGM$^{*}$ and dDGM architectures for OGB-Products.
    }
    
\scalebox{0.74}{
    \begin{tabular}{lcc cc}
    \toprule 
          & &
& 
         \textbf{dDGM$^{*}$} &  
         \textbf{dDGM}
         \\ \midrule

         
         
         No. Layer parameters & BatchNorm  & Activation & \multicolumn{2}{c}{Layer type}
         \\\hline
          (No. features, 32 per model space)  & Yes (dDGM$^{*}$)/ No (dDGM) & SiLU & Linear & Graph Conv 
          \\
          (32 per model space, 16 per model space) & Yes (dDGM$^{*}$)/ No (dDGM) & SiLU & Linear & Graph Conv 
          \\
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:dDGM_products}
\end{table*}

==> tables/heterophilic.tex <==



\begin{table*}[htbp!]
    \centering
    \caption{Results for  heterophilic datasets combining GCN diffusion layers with the dDGM$^{*}$ latent graph inference system. We display results using model spaces as well as product manifolds to construct the latent graphs.
    }
    
\scalebox{0.65}{
    \begin{tabular}{l cccc}
    \toprule 
         &

         \textbf{Texas} &  
         \textbf{Wisconsin} & 
         \textbf{Squirrel} &
         \textbf{Chameleon} 
         \\
         
         Homophily level &
         0.11 &
         0.21 &
         0.22 &
         0.23
         
          \\ 
         
         Nodes &
    
         183 &
         251 &
         5,201 &
           2,277
          \\
          
        Features &
   
         1,703 &
         1,703 &
         2,089 &
          2,325 
          \\
         
         Edges &
        
        295 &
         466 &
         198,498 &
         31,421 
          \\
         
         Classes &
      
        5 &
         5 &
         5 &
         5 \\
         
         Average Degree & 
      
        3.22 &
         3.71 &
         76.33 &
         27.60 \\
         
         $k$ & 
    
        2 &
         10 &
         3 &
         5 
         \\
         \midrule
         
         Model &
         \multicolumn{4}{c}{Accuracy $(\%)$ $\pm$ Standard Deviation}
         
          
         
         \\ 

        
        \midrule
         GCN-dDGM$^{*}$-E&
         $ \thirdd{80.00 {\scriptstyle \pm 8.31 }}$ &
         $ \thirdd{88.00 {\scriptstyle \pm 5.65}}$ &
         $ 34.35 {\scriptstyle \pm 2.34 }$ & 
         $ \first{48.90 {\scriptstyle \pm 3.61}}$ \\
         
        GCN-dDGM$^{*}$-H&
         $ 79.44 {\scriptstyle \pm 7.88}$ &
         $ \secondd{89.03 {\scriptstyle \pm 1.89 }}$ &
         $ \first{35.00 {\scriptstyle \pm 2.35}}$ & 
         $ 48.28 {\scriptstyle \pm 4.11 }$ \\
         
        GCN-dDGM$^{*}$-S&
         $ 73.88 {\scriptstyle \pm 9.95 }$ &
         $ 85.33 {\scriptstyle \pm 4.98 }$ &
         $ 33.12 {\scriptstyle \pm 2.22}$ & 
         $ \secondd{48.63{\scriptstyle \pm 3.12 }}$ \\ \midrule
         
        GCN-dDGM$^{*}$-HH&
         $ 78.89 {\scriptstyle \pm 8.53 }$ &
         $ \thirdd{88.00 {\scriptstyle \pm 3.26 }}$ &
         $ \thirdd{34.38 {\scriptstyle \pm 1.07}}$ & 
         $ \thirdd{48.33 {\scriptstyle \pm 4.14}}$ \\
         
        GCN-dDGM$^{*}$-SS&
         $ 73.89 {\scriptstyle \pm 8.62 }$ &
         $  74.66 {\scriptstyle \pm 18.85  }$ &
         $ 34.06 {\scriptstyle \pm 2.20 }$ & 
         $ 48.28 {\scriptstyle \pm 3.07}$ \\
         
         
        GCN-dDGM$^{*}$-EH&
         $ \first{81.67 {\scriptstyle \pm 7.05}}$ &
         $ 86.67 {\scriptstyle \pm 3.77}$ &
         $ 34.37 {\scriptstyle \pm 1.72}$ & 
         $ 47.58 {\scriptstyle \pm 3.85}$ \\
         
       GCN-dDGM$^{*}$-ES&
         $ \secondd{81.11 {\scriptstyle \pm 10.30}}$ &
         $ 76.00 {\scriptstyle \pm 11.31 }$ &
         $ 33.38 {\scriptstyle \pm 1.86}$ & 
         $ 47.49 {\scriptstyle \pm 3.60}$ \\
         
       GCN-dDGM$^{*}$-HS&
         $ \secondd{81.11 {\scriptstyle \pm 9.69}}$ &
         $ 86.67 {\scriptstyle \pm 1.89 }$ &
         $ \secondd{34.65 {\scriptstyle \pm 2.45}}$ & 
         $ 47.84 {\scriptstyle \pm 2.67}$ \\

        GCN-dDGM$^{*}$-EHH&
         $ \secondd{81.11 {\scriptstyle \pm 5.09}}$
          & $77.60 {\scriptstyle \pm 8.62}$
         &$33.19  {\scriptstyle \pm 1.92}$
         & $44.27 {\scriptstyle \pm 2.96}$ \\
         
       GCN-dDGM$^{*}$-EHS&
         $ 79.44 {\scriptstyle \pm 6.11}$ &
         $ \first{89.33 {\scriptstyle \pm 1.89 }}$ &
         $ 34.17 {\scriptstyle \pm 2.23}$ & 
         $ 47.58 {\scriptstyle \pm 4.54}$ \\
         
         
         \midrule

                  GCN-dDGM-E&
         $ 60.56 {\scriptstyle \pm 8.03}$ &
         $ 70.67 {\scriptstyle \pm 10.49 }$ &
         $ 29.87 {\scriptstyle \pm 2.46}$ & 
         $ 44.19 {\scriptstyle \pm 3.85}$ \\
         
        GCN-dDGM-H&
         $ 58.89 {\scriptstyle \pm 9.36}$ &
         $ 72.00 {\scriptstyle \pm 5.56}$ &
         $ 29.56 {\scriptstyle \pm 2.49}$ & 
         $ 44.01 {\scriptstyle \pm 4.08}$ \\
         
        GCN-dDGM-S&
         $ 59.44 {\scriptstyle \pm 8.62}$ &
         $ 62.66 {\scriptstyle \pm 16.11 }$ &
         $ 30.58 {\scriptstyle \pm 2.34}$ & 
         $ 45.46 {\scriptstyle \pm 2.35}$ \\ \midrule
         
        GCN-dDGM-HH&
         $ 57.22 {\scriptstyle \pm 5.58}$ &
         $ 60.00 {\scriptstyle \pm 19.87 }$ &
         $ 30.29 {\scriptstyle \pm 1.37}$ & 
         $ 44.19 {\scriptstyle \pm 3.78}$ \\
         
        GCN-dDGM-SS&
         $ 59.44 {\scriptstyle \pm 6.11}$ &
         $ 49.33 {\scriptstyle \pm 12.36}$ &
         $ 30.15 {\scriptstyle \pm 2.40}$ & 
         $ 45.29 {\scriptstyle \pm 1.87}$ \\
         
         
        GCN-dDGM-EH&
         $ 62.78 {\scriptstyle \pm 9.31}$ &
         $ 65.33  {\scriptstyle \pm 4.99 }$ &
         $ 30.00 {\scriptstyle \pm 2.58}$ & 
         $ 43.09 {\scriptstyle \pm 3.42}$ \\
         
       GCN-dDGM-ES&
         $ 60.56 {\scriptstyle \pm 8.03}$ &
         $ 69.33 {\scriptstyle \pm 6.80 }$ &
         $ 30.44 {\scriptstyle \pm 2.38}$ & 
         $ 45.68 {\scriptstyle \pm 2.66}$ \\
         
       GCN-dDGM-HS&
         $ 57.78 {\scriptstyle \pm 10.00}$ &
         $ 72.00  {\scriptstyle \pm 3.26 }$ &
         $ 30.06 {\scriptstyle \pm 2.66}$ & 
         $ 43.30 {\scriptstyle \pm 4.67}$ \\

        GCN-dDGM-EHH&
         $57.77 {\scriptstyle \pm 10.88}$
          & $44.80 {\scriptstyle \pm 10.55}$
         &$ 28.55 {\scriptstyle \pm 4.28}$
         & $41.01 {\scriptstyle \pm 7.68}$ \\
         
       GCN-dDGM-EHS&
         $ 58.89 {\scriptstyle \pm 7.53}$ &
         $ 76.00 {\scriptstyle \pm 3.26}$ &
         $ 30.27 {\scriptstyle \pm 2.95}$ & 
         $ 41.15 {\scriptstyle \pm 9.84}$ \\
         \midrule

         MLP$^{*}$ &
         $ 77.78 {\scriptstyle \pm 10.24}$ &
         $ 85.33 {\scriptstyle \pm 4.99}$ &
         $ 30.44 {\scriptstyle \pm 2.55}$ & 
         $ 40.35 {\scriptstyle \pm 3.37}$ \\ 
         
         GCN &
         $ 41.66 {\scriptstyle \pm 11.72}$ &
         $ 47.20 {\scriptstyle \pm 9.76}$ &
         $ 24.19 {\scriptstyle \pm 2.56}$ & 
         $ 32.56 {\scriptstyle \pm 3.53}$ \\

         
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:hetero_results_complete}
\end{table*}

==> tables/homophilic_extra1.tex <==


\begin{table*}[htbp!]
    \centering
    \caption[]{Results for classical homophilic datasets combining GCN diffusion layers with the dDGM$^{*}$ and dDGM latent graph inference system and using single model spaces to construct the latent graphs. 
    }
    
\scalebox{0.55}{
    \begin{tabular}{l cccccc}
    \toprule 
         &
         &
         \textbf{Cora} &  
         \textbf{CiteSeer} & 
         \textbf{PubMed} &
         \textbf{Physics} &
         \textbf{CS}
         \\
         
         Homophily level &
         &
         0.81 &
         0.74 &
         0.80 &
         0.93&
         0.80
         
          \\ 
         
         Nodes &
        &
         2,708 &
         3,327 &
         18,717 &
          34,493 &
          18,333
          \\
          
        Features &
        &
         1,433 &
         3,703 &
         500 &
          8,415 &
          6,805
          \\
         
         Edges &
        &
        5,278 &
         4,676 &
         44,327 &
         247,962 &
         81,894
          \\
         
         Classes &
        &
        7 &
         6 &
         3 &
         5 &
         15 \\
         
         Average Degree & 
        &
        3.9 &
         2.77 &
         4.5 &
         14.38 &
         8.93
         
          
         
         \\ 
         \midrule
         
         Model & $k$ &
         \multicolumn{5}{c}{Accuracy $(\%)$ $\pm$ Standard Deviation}
         
         \\

        
        \midrule
         GCN-dDGM$^{*}$-E& 3&
         $ \secondd{62.48 {\scriptstyle \pm 3.24}}$ &
         $ 62.47 {\scriptstyle \pm 3.20}$ &
         $ 83.89 {\scriptstyle \pm 0.70}$ & 
         $ 94.03 {\scriptstyle \pm 0.45}$ &
         $ 76.05 {\scriptstyle \pm 6.89}$\\
         
         GCN-dDGM$^{*}$-H & 3&
         $ \first{63.82 {\scriptstyle \pm 3.69 }}$ &
         $ \thirdd{63.76 {\scriptstyle \pm 3.40}}$ &
         $ \first{87.15 {\scriptstyle \pm 0.69}}$ & 
         $  93.24{\scriptstyle \pm 0.45 }$ &
         $  76.26{\scriptstyle \pm 6.39}$\\
         
         GCN-dDGM$^{*}$-S & 3&
         $ 32.78 {\scriptstyle \pm 5.90}$ &
         $ 21.96 {\scriptstyle \pm 6.32 }$ &
         $ 41.60 {\scriptstyle \pm 5.43}$ & 
         $  58.37 {\scriptstyle \pm 1.44}$ &
         $ 54.52 {\scriptstyle \pm 17.30}$\\
         
         

        
        \midrule
         GCN-dDGM$^{*}$-E & 5&
         $ 60.63 {\scriptstyle \pm 3.01 }$ &
         $ 63.28 {\scriptstyle \pm 3.35 }$ &
         $ \thirdd{86.82 {\scriptstyle \pm 0.69 }}$ & 
         $ \first{95.13 {\scriptstyle \pm 0.50}}$ &
         $ 80.46 {\scriptstyle \pm 2.34}$\\
         
         GCN-dDGM$^{*}$-H & 5&
         $ 61.48 {\scriptstyle \pm 3.68 }$ &
         $ \first{64.76 {\scriptstyle \pm 2.88}}$ &
         $ 85.00 {\scriptstyle \pm 0.69}$ & 
         $ 94.83 {\scriptstyle \pm 0.51}$ &
         $ 82.69 {\scriptstyle \pm 1.44}$\\
         
         GCN-dDGM$^{*}$-S & 5&
         $ 42.04 {\scriptstyle \pm 5.01 }$ &
         $ 22.20 {\scriptstyle \pm 6.23}$ &
         $ 40.38 {\scriptstyle \pm 5.44}$ & 
         $ 54.70 {\scriptstyle \pm 2.01}$ &
         $ 70.67 {\scriptstyle \pm 13.69}$\\
         
         
         
         \midrule
         GCN-dDGM$^{*}$-E & 7&
         $ \thirdd{62.30 {\scriptstyle \pm 5.27 }}$ &
         $ 61.36 {\scriptstyle \pm 7.46  }$ &
         $ \secondd{86.86 {\scriptstyle \pm 0.68 }}$ & 
         $ 93.71 {\scriptstyle \pm 3.23  }$ &
         $ \secondd{86.03 {\scriptstyle \pm 5.27 }}$\\
         
         GCN-dDGM$^{*}$-H & 7&
         $  61.44 {\scriptstyle \pm 10.83 }$ &
         $ 62.05 {\scriptstyle \pm 5.74 }$ &
         $ 85.19  {\scriptstyle \pm 5.07  }$ & 
         $ \secondd{95.05 {\scriptstyle \pm 0.30 }}$ &
         $ \thirdd{84.20 {\scriptstyle \pm 4.70 }}$\\
         
         GCN-dDGM$^{*}$-S & 7&
         $ 41.71 {\scriptstyle \pm 14.22 }$ &
         $ 20.75 {\scriptstyle \pm 2.84}$ &
         $ 40.49 {\scriptstyle \pm 1.57}$ & 
         $ 55.20 {\scriptstyle \pm 13.26 }$ & 
         $ 73.46 {\scriptstyle \pm 8.17}$\\
         
         
         
         \midrule
         GCN-dDGM$^{*}$-E & 10&
         $ 61.37 {\scriptstyle \pm 3.85 }$ &
         $ \secondd{64.27 {\scriptstyle \pm 3.97 }}$ &
         $ 85.48 {\scriptstyle \pm 4.40 }$ & 
         $ 91.82 {\scriptstyle \pm 3.62 }$ & 
         $ 81.42 {\scriptstyle \pm 4.60}$\\
         
         GCN-dDGM$^{*}$-H & 10&
         $ 61.63 {\scriptstyle \pm 4.56 }$ &
         $ 63.62 {\scriptstyle \pm 5.22}$ &
         $ 84.92 {\scriptstyle \pm 4.85 }$ & 
         $ \thirdd{95.02 {\scriptstyle \pm 0.46 }}$ &
         $ 80.36 {\scriptstyle \pm 5.42 }$\\
         
         GCN-dDGM$^{*}$-S & 10&
         $ 34.04 {\scriptstyle \pm 9.65}$ &
         $ 19.96 {\scriptstyle \pm 4.14}$ &
         $ 39.84 {\scriptstyle \pm 1.07}$ & 
         $ 50.52 {\scriptstyle \pm 2.77}$ & 
         $ 69.55 {\scriptstyle \pm 5.94 }$\\
         
         
         \midrule

         MLP$^{*}$ & N/A &
         $ 58.92 {\scriptstyle \pm 3.28}$ &
         $ 59.48 {\scriptstyle \pm 2.14}$ &
         $ 85.75{\scriptstyle \pm 1.02}$ & 
         $ 94.91 {\scriptstyle \pm 0.30}$ &  
         $  \first{87.80 {\scriptstyle \pm 1.54 }}$\\ 

         
               \midrule 
               
               &
         &
         \textbf{Cora} &  
         \textbf{CiteSeer} & 
         \textbf{PubMed} &
         \textbf{Physics} &
         \textbf{CS}
         \\
         \midrule
         GCN-dDGM-E & 3&
         $ 80.44 {\scriptstyle \pm 4.60 }$ &
         $ 70.18 {\scriptstyle \pm 1.46}$ &
         $ 87.45 {\scriptstyle \pm 0.72 }$ & 
         $ \secondd{96.03 {\scriptstyle \pm 0.41}}$ &
         $ 85.98 {\scriptstyle \pm 2.59}$
         \\
         
         GCN-dDGM-H & 3&
         $ 80.31 {\scriptstyle \pm 4.30 }$ &
         $ 69.78 {\scriptstyle \pm 1.56}$ &
         $ 85.79 {\scriptstyle \pm 0.73 }$ & 
         $ 95.29 {\scriptstyle \pm 0.43}$ &
         $ 85.95 {\scriptstyle \pm 2.58}$
         \\
         
         GCN-dDGM-S & 3&
         $ 73.26 {\scriptstyle \pm 4.33}$ &
         $ 67.98 {\scriptstyle \pm 2.21}$ &
         $ 81.39 {\scriptstyle \pm 1.00}$ & 
         $ 91.60 {\scriptstyle \pm 0.55 }$ &
         $ 76.76 {\scriptstyle \pm 4.65}$\\
         
        
         

        
        \midrule
         GCN-dDGM-E& 5&
         $ 82.74 {\scriptstyle \pm 4.42 }$ &
         $ 71.78 {\scriptstyle \pm 1.50}$ &
         $ \thirdd{87.60 {\scriptstyle \pm 0.69}}$ & 
         $ 95.96 {\scriptstyle \pm 0.40}$ &
         $ 87.88 {\scriptstyle \pm 2.55}$\\
         
         GCN-dDGM-H & 5&
         $ 80.80 {\scriptstyle \pm 4.43}$ &
         $ 67.53 {\scriptstyle \pm 2.12}$ &
         $ 87.58 {\scriptstyle \pm 0.71}$ & 
         $ \first{96.06 {\scriptstyle \pm 0.42}}$ &
         $ 87.65 {\scriptstyle \pm 2.56}$\\
         
         GCN-dDGM-S & 5&
         $  80.81{\scriptstyle \pm 2.30}$ &
         $ 71.81{\scriptstyle \pm 1.20}$ &
         $ 77.65{\scriptstyle \pm 1.01}$ & 
         $  95.91{\scriptstyle \pm 0.41 }$ &
         $ 80.73 {\scriptstyle \pm 4.62}$\\
         
         
         
         \midrule
         GCN-dDGM-E & 7&
         $ 82.11 {\scriptstyle \pm 4.24 }$ &
         $ \thirdd{72.35 {\scriptstyle \pm 1.92 }}$ &
         $ \secondd{87.69 {\scriptstyle \pm 0.67 }}$ & 
         $ 95.50 {\scriptstyle \pm 1.25 }$ &
         $ 87.17 {\scriptstyle \pm 3.82 }$\\
         
         GCN-dDGM-H & 7&
         $  \first{84.68 {\scriptstyle \pm 3.31 }}$ &
         $ 70.43 {\scriptstyle \pm 4.95 }$ &
         $ \first{87.74 {\scriptstyle \pm 0.72 }}$ & 
         $  \first{96.06 {\scriptstyle \pm 0.46 }}$ &
         $ \first{88.78 {\scriptstyle \pm 2.24 }}$\\
         
         GCN-dDGM-S & 7&
         $ 80.44 {\scriptstyle \pm 5.26}$ &
         $ \first{72.89 {\scriptstyle \pm 2.00 }}$ &
         $ 87.13 {\scriptstyle \pm 0.66 }$ & 
         $ 95.76 {\scriptstyle \pm 0.43 }$ & 
         $ 84.16 {\scriptstyle \pm 2.78 }$\\
         
      
         
         \midrule
         GCN-dDGM-E & 10&
         $ 81.67 {\scriptstyle \pm 5.74 }$ &
         $ \secondd{72.44 {\scriptstyle \pm 2.81 }}$ &
         $ 85.45 {\scriptstyle \pm 4.32 }$ & 
         $ \thirdd{95.99 {\scriptstyle \pm 0.49 }}$ &
         $ \thirdd{88.19 {\scriptstyle \pm 3.51}}$\\
         
         GCN-dDGM-H & 10&
         $ \secondd{83.15 {\scriptstyle \pm 3.20 }}$ &
         $ 71.54 {\scriptstyle \pm 1.46 }$ &
         $ \secondd{87.69 {\scriptstyle \pm 0.76 }}$ & 
         $ 95.84 {\scriptstyle \pm 0.73}$ &
         $ \secondd{88.49 {\scriptstyle \pm 2.21 }}$\\
         
         GCN-dDGM-S & 10&
         $ 82.70 {\scriptstyle \pm 3.22 }$ &
         $ 72.29 {\scriptstyle \pm 2.87 }$ &
         $ 87.38 {\scriptstyle \pm 0.69 }$ & 
         $  \secondd{96.03 {\scriptstyle \pm 0.44 }}$ & 
         $ 85.20 {\scriptstyle \pm 4.07 }$\\
         
        
         
         \midrule
         GCN & N/A &
         $ \thirdd{83.11 {\scriptstyle \pm 2.29}}$ &
         $ 69.97 {\scriptstyle \pm 2.06}$ &
         $ 85.75 {\scriptstyle \pm 1.01}$ & 
         $ 95.51 {\scriptstyle \pm 0.34}$ &
         $ 87.28 {\scriptstyle \pm 1.54 }$\\ 
         
\bottomrule
         
         
    \end{tabular}}
    
    \label{tab:homophilic_extra1}
\end{table*}

==> tables/homophilic_extra2.tex <==

\begin{table*}[htbp!]
    \centering
    \caption[Results for classical homophilic datasets combining GCN diffusion layers with the dDGM latent graph inference system and using single model spaces to construct the latent graphs. The dDGM uses the original dataset graph as inductive bias. Different $k$ values for the Gumbel Top-k trick are applied.]{Results for classical homophilic datasets combining GCN diffusion layers with the dDGM latent graph inference system and using single model spaces to construct the latent graphs. The dDGM uses the original dataset graph as inductive bias. Different $k$ values for the Gumbel Top-k trick are applied. Here, the GCN model, which leverages the dataset graph connectivity structure, is used as baseline.
    }
    
\scalebox{0.72}{
    \begin{tabular}{l cccccc}
    \toprule 
         &
         &
         \textbf{Cora} &  
         \textbf{CiteSeer} & 
         \textbf{PubMed} &
         \textbf{Physics} &
         \textbf{CS}
         \\
         
         Homophily level &
         &
         0.81 &
         0.74 &
         0.80 &
         0.93&
         0.80
         
          \\ 
         
         Nodes &
        &
         2,708 &
         3,327 &
         18,717 &
          34,493 &
          18,333
          \\
          
        Features &
        &
         1,433 &
         3,703 &
         500 &
          8,415 &
          6,805
          \\
         
         Edges &
        &
        5,278 &
         4,676 &
         44,327 &
         247,962 &
         81,894
          \\
         
         Classes &
        &
        7 &
         6 &
         3 &
         5 &
         15 \\
         
         Average Degree & 
        &
        3.9 &
         2.77 &
         4.5 &
         14.38 &
         8.93
         
          
         
         \\ 
         \midrule
         
         Model & $k$ &
         \multicolumn{5}{c}{Accuracy $(\%)$ $\pm$ Standard Deviation}
         
         \\
          \midrule
         GCN-dDGM-E & 3&
         $ 80.44 {\scriptstyle \pm 4.60 }$ &
         $ 70.18 {\scriptstyle \pm 1.46}$ &
         $ 87.45 {\scriptstyle \pm 0.72 }$ & 
         $ \secondd{96.03 {\scriptstyle \pm 0.41}}$ &
         $ 85.98 {\scriptstyle \pm 2.59}$
         \\
         
         GCN-dDGM-H & 3&
         $ 80.31 {\scriptstyle \pm 4.30 }$ &
         $ 69.78 {\scriptstyle \pm 1.56}$ &
         $ 85.79 {\scriptstyle \pm 0.73 }$ & 
         $ 95.29 {\scriptstyle \pm 0.43}$ &
         $ 85.95 {\scriptstyle \pm 2.58}$
         \\
         
         GCN-dDGM-S & 3&
         $ 73.26 {\scriptstyle \pm 4.33}$ &
         $ 67.98 {\scriptstyle \pm 2.21}$ &
         $ 81.39 {\scriptstyle \pm 1.00}$ & 
         $ 91.60 {\scriptstyle \pm 0.55 }$ &
         $ 76.76 {\scriptstyle \pm 4.65}$\\
         
        
         

        
        \midrule
         GCN-dDGM-E& 5&
         $ 82.74 {\scriptstyle \pm 4.42 }$ &
         $ 71.78 {\scriptstyle \pm 1.50}$ &
         $ \thirdd{87.60 {\scriptstyle \pm 0.69}}$ & 
         $ 95.96 {\scriptstyle \pm 0.40}$ &
         $ 87.88 {\scriptstyle \pm 2.55}$\\
         
         GCN-dDGM-H & 5&
         $ 80.80 {\scriptstyle \pm 4.43}$ &
         $ 67.53 {\scriptstyle \pm 2.12}$ &
         $ 87.58 {\scriptstyle \pm 0.71}$ & 
         $ \first{96.06 {\scriptstyle \pm 0.42}}$ &
         $ 87.65 {\scriptstyle \pm 2.56}$\\
         
         GCN-dDGM-S & 5&
         $  80.81{\scriptstyle \pm 2.30}$ &
         $ 71.81{\scriptstyle \pm 1.20}$ &
         $ 77.65{\scriptstyle \pm 1.01}$ & 
         $  95.91{\scriptstyle \pm 0.41 }$ &
         $ 80.73 {\scriptstyle \pm 4.62}$\\
         
         
         
         \midrule
         GCN-dDGM-E & 7&
         $ 82.11 {\scriptstyle \pm 4.24 }$ &
         $ \thirdd{72.35 {\scriptstyle \pm 1.92 }}$ &
         $ \secondd{87.69 {\scriptstyle \pm 0.67 }}$ & 
         $ 95.50 {\scriptstyle \pm 1.25 }$ &
         $ 87.17 {\scriptstyle \pm 3.82 }$\\
         
         GCN-dDGM-H & 7&
         $  \first{84.68 {\scriptstyle \pm 3.31 }}$ &
         $ 70.43 {\scriptstyle \pm 4.95 }$ &
         $ \first{87.74 {\scriptstyle \pm 0.72 }}$ & 
         $  \first{96.06 {\scriptstyle \pm 0.46 }}$ &
         $ \first{88.78 {\scriptstyle \pm 2.24 }}$\\
         
         GCN-dDGM-S & 7&
         $ 80.44 {\scriptstyle \pm 5.26}$ &
         $ \first{72.89 {\scriptstyle \pm 2.00 }}$ &
         $ 87.13 {\scriptstyle \pm 0.66 }$ & 
         $ 95.76 {\scriptstyle \pm 0.43 }$ & 
         $ 84.16 {\scriptstyle \pm 2.78 }$\\
         
      
         
         \midrule
         GCN-dDGM-E & 10&
         $ 81.67 {\scriptstyle \pm 5.74 }$ &
         $ \secondd{72.44 {\scriptstyle \pm 2.81 }}$ &
         $ 85.45 {\scriptstyle \pm 4.32 }$ & 
         $ \thirdd{95.99 {\scriptstyle \pm 0.49 }}$ &
         $ \thirdd{88.19 {\scriptstyle \pm 3.51}}$\\
         
         GCN-dDGM-H & 10&
         $ \secondd{83.15 {\scriptstyle \pm 3.20 }}$ &
         $ 71.54 {\scriptstyle \pm 1.46 }$ &
         $ \secondd{87.69 {\scriptstyle \pm 0.76 }}$ & 
         $ 95.84 {\scriptstyle \pm 0.73}$ &
         $ \secondd{88.49 {\scriptstyle \pm 2.21 }}$\\
         
         GCN-dDGM-S & 10&
         $ 82.70 {\scriptstyle \pm 3.22 }$ &
         $ 72.29 {\scriptstyle \pm 2.87 }$ &
         $ 87.38 {\scriptstyle \pm 0.69 }$ & 
         $  \secondd{96.03 {\scriptstyle \pm 0.44 }}$ & 
         $ 85.20 {\scriptstyle \pm 4.07 }$\\
         
        
         
         \midrule
         GCN & N/A &
         $ \thirdd{83.11 {\scriptstyle \pm 2.29}}$ &
         $ 69.97 {\scriptstyle \pm 2.06}$ &
         $ 85.75 {\scriptstyle \pm 1.01}$ & 
         $ 95.51 {\scriptstyle \pm 0.34}$ &
         $ 87.28 {\scriptstyle \pm 1.54 }$\\ 
         

         
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:homophilic_extra2}
\end{table*}

==> tables/homophilic_extra3.tex <==


\begin{table*}[htbp!]
    \centering
    \caption{Results for classical homophilic datasets combining GCN diffusion layers with the dDGM$^{*}$ module and using product manifolds to construct the latent graphs.}
    
\scalebox{0.65}{
    \begin{tabular}{l cccccc}
    \toprule 
         &
         &
         \textbf{Cora} &  
         \textbf{CiteSeer} & 
         \textbf{PubMed} &
         \textbf{Physics} &
         \textbf{CS}

         \\
         
         Homophily level &
         &
         0.81 &
         0.74 &
         0.80 &
         0.93&
         0.80
         
          \\ 
         
         Nodes &
        &
         2,708 &
         3,327 &
         18,717 &
          34,493 &
          18,333
          \\
          
        Features &
        &
         1,433 &
         3,703 &
         500 &
          8,415 &
          6,805
          \\
         
         Edges &
        &
        5,278 &
         4,676 &
         44,327 &
         247,962 &
         81,894
          \\
         
         Classes &
        &
        7 &
         6 &
         3 &
         5 &
         15 \\
         
         Average Degree & 
        &
        3.9 &
         2.77 &
         4.5 &
         14.38 &
         8.93
         
          
         
         \\ 
         \midrule
         
         Model & $k$ &
         \multicolumn{5}{c}{Accuracy $(\%)$ $\pm$ Standard Deviation}
         
         \\

        
        \midrule

         
         GCN-dDGM$^{*}$-HH & 3&
         $ 57.00 {\scriptstyle \pm 9.78 }$ &
         $ 62.50 {\scriptstyle \pm 4.25 }$ &
         $ \first{87.43 {\scriptstyle \pm 0.40}}$ & 
         $ 92.20 {\scriptstyle \pm 3.47}$ &
         $ 74.88 {\scriptstyle \pm 4.65}$\\
         
         GCN-dDGM$^{*}$-SS & 3&
         $ 38.26 {\scriptstyle \pm 10.94}$ &
         $ 24.20 {\scriptstyle \pm 10.12}$ &
         $ 41.59 {\scriptstyle \pm 0.71}$ & 
         $ 54.43 {\scriptstyle \pm 10.00}$ &
         $ 55.29 {\scriptstyle \pm 7.33 }$\\
         
         GCN-dDGM$^{*}$-EH & 3&
         $ 61.07 {\scriptstyle \pm 10.18}$ &
         $ 65.13 {\scriptstyle \pm 2.19 }$ &
         $ 86.67 {\scriptstyle \pm 0.69 }$ & 
         $ 94.85 {\scriptstyle \pm 0.55 }$ & 
         $ 85.91 {\scriptstyle \pm 2.88}$\\
         
         
         GCN-dDGM$^{*}$-ES & 3&
         $ 62.07 {\scriptstyle \pm 4.08 }$ &
         $ 64.31  {\scriptstyle \pm 3.15 }$ &
         $ 86.85  {\scriptstyle \pm 1.02 }$ & 
         $ 95.01 {\scriptstyle \pm 0.55 }$ & 
         $ 78.67  {\scriptstyle \pm 4.44 }$\\
         
         GCN-dDGM$^{*}$-HS & 3&
         $ 59.55 {\scriptstyle \pm 10.90 }$ &
         $  63.95 {\scriptstyle \pm 2.35 }$ &
         $ \secondd{87.04 {\scriptstyle \pm 0.79} }$ & 
         $ 95.02 {\scriptstyle \pm 0.45 }$ & 
         $ 76.55 {\scriptstyle \pm 9.89}$\\

         GCN-dDGM$^{*}$-EHH & 3&
         $ \first{70.85 {\scriptstyle \pm 4.30} }$ &
         $ \first{68.86 {\scriptstyle \pm 2.97} }$ &
         $  39.93 {\scriptstyle \pm 1.35 }$ & 
         $ \secondd{95.21 {\scriptstyle \pm 0.34} }$ & 
         $  \first{92.22  {\scriptstyle \pm 1.09} }$\\
         
         GCN-dDGM$^{*}$-EHS & 3&
         $ 66.87 {\scriptstyle \pm 3.27 }$ &
         $  63.80 {\scriptstyle \pm 2.94 }$ &
         $ \thirdd{87.03  {\scriptstyle \pm 0.70 }}$ & 
         $ 95.03 {\scriptstyle \pm 0.39}$ & 
         $  88.64 {\scriptstyle \pm 1.90}$\\

         
         

        
        \midrule

         
         GCN-dDGM$^{*}$-HH & 5&
         $ 59.03 {\scriptstyle \pm 4.86}$ &
         $ 63.47 {\scriptstyle \pm 1.70}$ &
         $ 86.30 {\scriptstyle \pm 0.99}$ & 
         $ 94.31 {\scriptstyle \pm 0.47 }$ &
         $ 76.48  {\scriptstyle \pm 4.30 }$\\
         
         GCN-dDGM$^{*}$-SS & 5&
         $ 41.33 {\scriptstyle \pm 10.54 }$ &
         $  21.48 {\scriptstyle \pm 3.81 }$ &
         $ 40.70 {\scriptstyle \pm 1.31 }$ & 
         $ 53.43 {\scriptstyle \pm 9.15 }$ &
         $ 58.47  {\scriptstyle \pm 5.79 }$\\
         
         GCN-dDGM$^{*}$-EH & 5&
         $ 63.67 {\scriptstyle \pm 6.48 }$ &
         $ 61.59  {\scriptstyle \pm 12.28 }$ &
         $ 86.90 {\scriptstyle \pm 1.16 }$ & 
         $ 93.94 {\scriptstyle \pm 3.37}$ & 
         $  86.00 {\scriptstyle \pm 3.04 }$\\
         
         
         GCN-dDGM$^{*}$-ES & 5&
         $ 63.44 {\scriptstyle \pm 4.18 }$ &
         $  63.10 {\scriptstyle \pm 2.71 }$ &
         $  86.83 {\scriptstyle \pm 0.82 }$ & 
         $ 93.92 {\scriptstyle \pm 2.38 }$ &
         $ 75.86 {\scriptstyle \pm 11.18 }$\\
         
         GCN-dDGM$^{*}$-HS & 5&
         $ 64.44 {\scriptstyle \pm 4.00 }$ &
         $ 62.80 {\scriptstyle \pm 3.90 }$ &
         $ 85.17 {\scriptstyle \pm 4.72 }$ & 
         $ 94.81 {\scriptstyle \pm 0.23}$ & 
         $ 77.93 {\scriptstyle \pm 4.47 }$\\

         GCN-dDGM$^{*}$-EHH & 5&
         $ \thirdd{69.74 {\scriptstyle \pm 5.09 }}$ &
         $ \secondd{66.81 {\scriptstyle \pm 2.04  }}$ &
         $  39.93 {\scriptstyle \pm 1.35 }$ & 
         $ \first{95.25 {\scriptstyle \pm 0.36 }}$ & 
         $  \thirdd{90.46 {\scriptstyle \pm 1.03 }}$\\
         
         GCN-dDGM$^{*}$-EHS & 5&
         $ 64.82 {\scriptstyle \pm 3.68 }$ &
         $  64.62 {\scriptstyle \pm 3.35}$ &
         $ 86.85  {\scriptstyle \pm 0.97 }$ & 
         $ 94.30 {\scriptstyle \pm 2.09 }$ & 
         $ 88.48 {\scriptstyle \pm 1.77 }$\\

         
         
         \midrule

         
         GCN-dDGM$^{*}$-HH & 7&
         $ 54.58  {\scriptstyle \pm 10.40 }$ &
         $ 62.02 {\scriptstyle \pm 5.73 }$ &
         $  86.91 {\scriptstyle \pm 0.89 }$ & 
         $  94.08 {\scriptstyle \pm 3.14 }$ & 
         $ 79.88 {\scriptstyle \pm 5.77 }$\\
         
         GCN-dDGM$^{*}$-SS & 7&
         $ 40.22 {\scriptstyle \pm 13.00}$ &
         $ 20.54 {\scriptstyle \pm 3.42 }$ &
         $ 40.49 {\scriptstyle \pm 1.39 }$ & 
         $ 58.67  {\scriptstyle \pm 16.44}$ & 
         $ 50.94 {\scriptstyle \pm 14.36}$\\
         
         GCN-dDGM$^{*}$-EH & 7&
         $ 59.92 {\scriptstyle \pm 8.92 }$ &
         $ 64.79 {\scriptstyle \pm 2.32}$ &
         $ 86.97 {\scriptstyle \pm 0.45 }$ & 
         $ 94.18 {\scriptstyle \pm 2.46 }$ & 
         $ 80.82 {\scriptstyle \pm 6.38}$\\
         
         
         GCN-dDGM$^{*}$-ES & 7&
         $ 61.44 {\scriptstyle \pm 3.23 }$ &
         $  62.41 {\scriptstyle \pm 2.88 }$ &
         $  86.48 {\scriptstyle \pm 0.58 }$ & 
         $ 92.13 {\scriptstyle \pm 5.81 }$ & 
         $ 74.84 {\scriptstyle \pm 7.24 }$\\
         
         GCN-dDGM$^{*}$-HS & 7&
         $ 59.11 {\scriptstyle \pm 8.15 }$ &
         $ 64.86 {\scriptstyle \pm 3.03}$ &
         $ 85.21 {\scriptstyle \pm 4.74 }$ & 
         $ 94.72 {\scriptstyle \pm 0.92 }$ &
         $ 83.23 {\scriptstyle \pm 3.95 }$\\

         GCN-dDGM$^{*}$-EHH & 7&
         $ \secondd{70.37 {\scriptstyle \pm  4.72} }$ &
         $ 62.50 {\scriptstyle \pm 11.69 }$ &
         $ 39.93  {\scriptstyle \pm 1.35 }$ & 
         $ \thirdd{95.16 {\scriptstyle \pm 0.37} }$ & 
         $ \secondd{91.58 {\scriptstyle \pm 0.91 }}$\\
         
         GCN-dDGM$^{*}$-EHS & 7&
         $ 63.30 {\scriptstyle \pm 3.93 }$ &
         $ 64.54  {\scriptstyle \pm 1.89 }$ &
         $ 86.99  {\scriptstyle \pm 0.79 }$ & 
         $ 92.85 {\scriptstyle \pm 2.49 }$ &
         $ 86.96 {\scriptstyle \pm 2.54}$\\

         
         
         \midrule
         
         GCN-dDGM$^{*}$-HH & 10&
         $ 57.59 {\scriptstyle \pm 8.05}$ &
         $ 59.43 {\scriptstyle \pm 5.46}$ &
         $ 86.43 {\scriptstyle \pm 0.70}$ & 
         $ 92.50 {\scriptstyle \pm 3.35}$ & 
         $  73.13 {\scriptstyle \pm 8.55}$\\
         
         GCN-dDGM$^{*}$-SS & 10&
         $ 36.30 {\scriptstyle \pm 8.23}$ &
         $ 21.20 {\scriptstyle \pm 2.88 }$ &
         $ 39.83 {\scriptstyle \pm 1.17}$ & 
         $ 50.52 {\scriptstyle \pm 2.77}$ & 
         $ 53.85 {\scriptstyle \pm 16.78}$\\
         
         GCN-dDGM$^{*}$-EH & 10&
         $ 59.63 {\scriptstyle \pm 11.04 }$ &
         $ \thirdd{65.49 {\scriptstyle \pm 2.86 }}$ &
         $ 84.54 {\scriptstyle \pm 5.77 }$ & 
         $ 93.55 {\scriptstyle \pm 4.53 }$ & 
         $ 72.79 {\scriptstyle \pm 5.79 }$\\
         
         
         GCN-dDGM$^{*}$-ES & 10&
         $ 63.04 {\scriptstyle \pm 4.21}$ &
         $ 62.65  {\scriptstyle \pm 6.29 }$ &
         $  86.71 {\scriptstyle \pm 0.89 }$ & 
         $ 93.42 {\scriptstyle \pm 3.22 }$ & 
         $ 74.85 {\scriptstyle \pm 7.59 }$\\
         
         GCN-dDGM$^{*}$-HS & 10&
         $ 64.24 {\scriptstyle \pm 5.38 }$ &
         $ 62.73 {\scriptstyle \pm 2.59 }$ &
         $ 85.24 {\scriptstyle \pm 4.58 }$ & 
         $ 95.03 {\scriptstyle \pm 0.64 }$ & 
         $ 75.03 {\scriptstyle \pm 6.18 }$\\

         GCN-dDGM$^{*}$-EHH & 10&
         $ 69.63 {\scriptstyle \pm 4.00 }$ &
         $ 64.70 {\scriptstyle \pm 4.61 }$ &
         $  39.93 {\scriptstyle \pm 1.35 }$ & 
         $ 95.02 {\scriptstyle \pm 0.39}$ & 
         $  83.81 {\scriptstyle \pm 11.41}$\\
         
         GCN-dDGM$^{*}$-EHS & 10&
         $ 63.61 {\scriptstyle \pm 3.71 }$ &
         $  64.52 {\scriptstyle \pm 2.77 }$ &
         $ 86.60  {\scriptstyle \pm 0.66}$ & 
         $ 90.03 {\scriptstyle \pm 4.86 }$ & 
         $ 84.52 {\scriptstyle \pm 7.39 }$\\

         

         
         \midrule

         MLP$^{*}$ & N/A &
         $ 58.92 {\scriptstyle \pm 3.28}$ &
         $ 59.48 {\scriptstyle \pm 2.14}$ &
         $ 85.75{\scriptstyle \pm 1.02}$ & 
         $ 94.91 {\scriptstyle \pm 0.30}$ &  
         $  87.80 {\scriptstyle \pm 1.54 }$\\ 

         
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:homophilic_extra3}
\end{table*}

==> tables/homophilic_extra4.tex <==


\begin{table*}[htbp!]
    \centering
    \caption{Results for classical homophilic datasets combining GCN diffusion layers with the dDGM module and using product manifold to construct the latent graphs.}
    
\scalebox{0.65}{
    \begin{tabular}{l cccccc}
    \toprule 
         &
         &
         \textbf{Cora} &  
         \textbf{CiteSeer} & 
         \textbf{PubMed} &
         \textbf{Physics} &
         \textbf{CS}
         \\
         
         Homophily level &
         &
         0.81 &
         0.74 &
         0.80 &
         0.93&
         0.80
         
          \\ 
         
         Nodes &
        &
         2,708 &
         3,327 &
         18,717 &
          34,493 &
          18,333
          \\
          
        Features &
        &
         1,433 &
         3,703 &
         500 &
          8,415 &
          6,805
          \\
         
         Edges &
        &
        5,278 &
         4,676 &
         44,327 &
         247,962 &
         81,894
          \\
         
         Classes &
        &
        7 &
         6 &
         3 &
         5 &
         15 \\
         
         Average Degree & 
        &
        3.9 &
         2.77 &
         4.5 &
         14.38 &
         8.93
         
          
         
         \\ 
         \midrule
         
         Model & $k$ &
         \multicolumn{5}{c}{Accuracy $(\%)$ $\pm$ Standard Deviation}
         
         \\
          \midrule

         
         GCN-dDGM-HH & 3&
         $ 77.82 {\scriptstyle \pm 5.46 }$ &
         $ 71.27 {\scriptstyle \pm 2.09 }$ &
         $ 87.35 {\scriptstyle \pm 0.65 }$ & 
         $ 94.04 {\scriptstyle \pm 3.54 }$ &
         $ 82.91 {\scriptstyle \pm 3.00}$\\
         
         GCN-dDGM-SS & 3&
         $ 67.00 {\scriptstyle \pm 10.23}$ &
         $ 59.16 {\scriptstyle \pm 5.96}$ &
         $ 86.83 {\scriptstyle \pm 0.60}$ & 
         $ 90.30 {\scriptstyle \pm 5.90}$ &
         $ 59.31 {\scriptstyle \pm 7.18}$\\
         
         GCN-dDGM-EH & 3&
         $ 83.65 {\scriptstyle \pm 5.25 }$ &
         $ 72.89 {\scriptstyle \pm 1.64}$ &
         $ 87.62 {\scriptstyle \pm  0.64}$ & 
         $ 96.07 {\scriptstyle \pm 0.27}$ & 
         $ 91.37 {\scriptstyle \pm 1.28}$\\
         
         
         GCN-dDGM-ES & 3&
         $ 81.19 {\scriptstyle \pm 6.63}$ &
         $ 71.87  {\scriptstyle \pm 3.20 }$ &
         $  86.47 {\scriptstyle \pm 2.30 }$ & 
         $  95.32 {\scriptstyle \pm 0.42 }$ & 
         $ 90.87 {\scriptstyle \pm 0.82 }$\\
         
         GCN-dDGM-HS & 3&
         $ 80.70 {\scriptstyle \pm 2.96 }$ &
         $ 72.77 {\scriptstyle \pm 2.76}$ &
         $ 87.29 {\scriptstyle \pm 0.85 }$ & 
         $ 96.10 {\scriptstyle \pm 0.35}$ & 
         $  89.43 {\scriptstyle \pm 2.37}$\\

         GCN-dDGM-EHH & 3&
         $ \secondd{86.59 {\scriptstyle \pm 3.33}}$ &
         $ \first{75.42 {\scriptstyle \pm 2.39 }}$ &
         $  49.17 {\scriptstyle \pm 19.39 }$ & 
         $ 96.06 {\scriptstyle \pm 0.34}$ & 
         $  \first{92.86 {\scriptstyle \pm 0.96} }$\\
         
         GCN-dDGM-EHS & 3&
         $ \thirdd{85.84 {\scriptstyle \pm 2.96 }}$ &
         $  69.98 {\scriptstyle \pm 2.70}$ &
         $ 87.35  {\scriptstyle \pm 0.90 }$ & 
         $ 95.96 {\scriptstyle \pm 0.42 }$ & 
         $ 89.93 {\scriptstyle \pm 3.86}$\\
         

        
        \midrule

         
         GCN-dDGM-HH & 5&
         $ 76.09 {\scriptstyle \pm 7.11 }$ &
         $ 72.65 {\scriptstyle \pm 2.23 }$ &
         $ 87.36 {\scriptstyle \pm 0.78 }$ & 
         $  95.93 {\scriptstyle \pm 0.37 }$ &
         $  80.73 {\scriptstyle \pm 4.62 }$\\
         
         GCN-dDGM-SS & 5&
         $ 65.96 {\scriptstyle \pm 9.46}$ &
         $ 65.37 {\scriptstyle \pm 5.90 }$ &
         $ 87.21 {\scriptstyle \pm 0.75 }$ & 
         $ 90.40 {\scriptstyle \pm 6.90 }$ &
         $ 70.60 {\scriptstyle \pm 9.31}$\\
         
         GCN-dDGM-EH & 5&
         $ 82.32 {\scriptstyle \pm 4.71 }$ &
         $ 73.56 {\scriptstyle \pm 2.75 }$ &
         $ \thirdd{87.67 {\scriptstyle \pm 0.76}}$ & 
         $ 94.48 {\scriptstyle \pm 4.33}$ & 
         $ 91.11 {\scriptstyle \pm 1.57 }$\\
         
         
         GCN-dDGM-ES & 5&
         $ 81.44 {\scriptstyle \pm 5.80 }$ &
         $  71.57 {\scriptstyle \pm 2.08 }$ &
         $  87.41 {\scriptstyle \pm 1.14 }$ & 
         $ 96.11 {\scriptstyle \pm 0.40 }$ &
         $ 89.31 {\scriptstyle \pm 2.31 }$\\
         
         GCN-dDGM-HS & 5&
         $ 82.59 {\scriptstyle \pm 4.50}$ &
         $ 72.51 {\scriptstyle \pm 2.52 }$ &
         $ \secondd{87.79 {\scriptstyle \pm 1.08 }}$ & 
         $ 95.13 {\scriptstyle \pm 2.41 }$ & 
         $ 90.98 {\scriptstyle \pm 1.00 }$\\

         GCN-dDGM-EHH & 5&
         $ \first{86.63 {\scriptstyle \pm 3.25 }}$ &
         $ 73.95 {\scriptstyle \pm 2.97 }$ &
         $ 44.53  {\scriptstyle \pm 13.84 }$ & 
         $ 96.16 {\scriptstyle \pm 0.37 }$ & 
         $ \secondd{92.30  {\scriptstyle \pm 1.05}}$\\
         
         GCN-dDGM-EHS & 5&
         $ 83.58 {\scriptstyle \pm 4.39 }$ &
         $  74.00 {\scriptstyle \pm 1.68 }$ &
         $ 87.12  {\scriptstyle \pm 0.72 }$ & 
         $ \thirdd{96.17 {\scriptstyle \pm 0.30} }$ & 
         $ \thirdd{92.06 {\scriptstyle \pm 0.83}}$\\
         
         \midrule

         
         GCN-dDGM-HH & 7&
         $  79.70 {\scriptstyle \pm 5.55 }$ &
         $ 71.30 {\scriptstyle \pm 2.94 }$ &
         $ 85.08 {\scriptstyle \pm 5.15}$ & 
         $ 95.99 {\scriptstyle \pm 0.44 }$ & 
         $ 86.27 {\scriptstyle \pm 2.66 }$\\
         
         GCN-dDGM-SS & 7&
         $ 63.62 {\scriptstyle \pm 9.19 }$ &
         $ 61.39 {\scriptstyle \pm 5.61 }$ &
         $ 87.41 {\scriptstyle \pm 0.55 }$ & 
         $ 91.68 {\scriptstyle \pm 5.50 }$ & 
         $ 64.05 {\scriptstyle \pm 13.45 }$\\
         
         GCN-dDGM-EH & 7&
         $ 82.89 {\scriptstyle \pm 4.31 }$ &
         $ 71.84 {\scriptstyle \pm 2.50 }$ &
         $ 87.40 {\scriptstyle \pm 0.59 }$ & 
         $ 96.06 {\scriptstyle \pm 0.52 }$ & 
         $ 91.22 {\scriptstyle \pm 0.93 }$\\
         
         
         GCN-dDGM-ES & 7&
         $ 80.85 {\scriptstyle \pm 4.75}$ &
         $  71.08 {\scriptstyle \pm 4.14 }$ &
         $  85.54 {\scriptstyle \pm 5.04 }$ & 
         $ 95.24 {\scriptstyle \pm 2.88}$ & 
         $ 89.21 {\scriptstyle \pm 2.56 }$\\
         
         GCN-dDGM-HS & 7&
         $ 81.78 {\scriptstyle \pm 5.25 }$ &
         $ 72.41 {\scriptstyle \pm 1.86}$ &
         $ 87.27 {\scriptstyle \pm 0.62 }$ & 
         $ 96.03 {\scriptstyle \pm 0.37 }$ &
         $ 89.90 {\scriptstyle \pm 1.06}$\\

         GCN-dDGM-EHH & 7&
         $ 85.65 {\scriptstyle \pm 3.54 }$ &
         $ \secondd{74.67 {\scriptstyle \pm 2.01 }}$ &
         $  48.04 {\scriptstyle \pm  16.30 }$ & 
         $ \secondd{96.18 {\scriptstyle \pm 0.39 }}$ & 
         $  90.74 {\scriptstyle \pm 2.88 }$\\
         
         GCN-dDGM-EHS & 7&
         $ 83.70 {\scriptstyle \pm 3.88 }$ &
         $ 73.02  {\scriptstyle \pm 2.57}$ &
         $  87.61 {\scriptstyle \pm 0.67 }$ & 
         $ 96.09 {\scriptstyle \pm 0.38 }$ &
         $ 90.64 {\scriptstyle \pm 1.26}$\\
         
         \midrule
         
         GCN-dDGM-HH& 10&
         $ 82.18 {\scriptstyle \pm 2.90 }$ &
         $ 72.47 {\scriptstyle \pm 2.81 }$ &
         $ 87.50 {\scriptstyle \pm 0.91 }$ & 
         $ 94.73 {\scriptstyle \pm 2.83 }$ & 
         $ 86.48 {\scriptstyle \pm 0.88 }$\\
         
         GCN-dDGM-SS & 10&
         $ 66.15 {\scriptstyle \pm 1.61}$ &
         $ 61.51 {\scriptstyle \pm 8.14 }$ &
         $ \first{87.82 {\scriptstyle \pm 0.59} }$ & 
         $ 90.72 {\scriptstyle \pm 5.26 }$ & 
         $ 69.62 {\scriptstyle \pm 10.14 }$\\
         
         GCN-dDGM-EH & 10&
         $ 81.44 {\scriptstyle \pm 3.94 }$ &
         $ 73.10 {\scriptstyle \pm 2.26 }$ &
         $ 87.41 {\scriptstyle \pm 0.80 }$ & 
         $ 96.03 {\scriptstyle \pm 0.37 }$ & 
         $ 90.98 {\scriptstyle \pm 1.15 }$\\
         
         
         GCN-dDGM-ES & 10&
         $ 80.07 {\scriptstyle \pm 5.40}$ &
         $  72.86 {\scriptstyle \pm 2.51 }$ &
         $  87.50 {\scriptstyle \pm 0.65}$ & 
         $ 95.41 {\scriptstyle \pm 1.73 }$ & 
         $ 90.25 {\scriptstyle \pm 1.79}$\\
         
         GCN-dDGM-HS & 10&
         $ 83.78 {\scriptstyle \pm 3.32}$ &
         $ 72.52 {\scriptstyle \pm 2.82}$ &
         $ 85.89 {\scriptstyle \pm 4.29}$ & 
         $ 95.84 {\scriptstyle \pm 0.29}$ & 
         $ 88.64 {\scriptstyle \pm 2.97}$\\

         GCN-dDGM-EHH & 10&
         $  84.53 {\scriptstyle \pm 3.84 }$ &
         $\thirdd{ 74.33 {\scriptstyle \pm 2.30 }}$ &
         $ 39.93 {\scriptstyle \pm 1.35  }$ & 
         $ 95.63 {\scriptstyle \pm 1.36  }$ & 
         $ 91.54 {\scriptstyle \pm 2.09 }$\\
         
         GCN-dDGM-EHS& 10&
         $ 83.50 {\scriptstyle \pm 4.64}$ &
         $  71.82 {\scriptstyle \pm 1.68}$ &
         $  87.05 {\scriptstyle \pm 1.38}$ & 
         $ \first{96.21 {\scriptstyle \pm 0.44}}$ & 
         $ 91.42 {\scriptstyle \pm 1.08}$\\
         
         \midrule
         GCN & N/A &
         $ 83.11 {\scriptstyle \pm 2.29}$ &
         $ 69.97 {\scriptstyle \pm 2.06}$ &
         $ 85.75 {\scriptstyle \pm 1.01}$ & 
         $ 95.51 {\scriptstyle \pm 0.34}$ &
         $ 87.28 {\scriptstyle \pm 1.54 }$\\ 
         

         
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:homophilic_extra4}
\end{table*}

==> tables/homophily_learning.tex <==


\begin{table*}[htbp!]
    \centering
    \caption{Homophily level of the learned latent graphs. Latent graph inference modules which use different manifolds to generate their respective latent graphs achieve different homophily levels. Also, depending on weight initialization, the inference system can converge to slightly different latent graphs.
    }
    
\scalebox{0.55}{
    \begin{tabular}{l cccc}
    \toprule 
         &

         \textbf{Texas} &  
         \textbf{Wisconsin} & 
         \textbf{Squirrel} &
         \textbf{Chameleon} 
         \\
         
         Original Graph Homophily &
         0.11 &
         0.21 &
         0.22 &
         0.23
         
         \\ 
                  $k$ & 
    
        2 &
         10 &
         3 &
         5 
         \\
         
         \midrule
         
         Model &
         \multicolumn{4}{c}{Latent Graph Homophily $h$ $\pm$ Standard Deviation}
         
         \\

        
        \midrule
         GCN-dDGM$^{*}$-E&
         $ 0.89 {\scriptstyle \pm 0.02 }$ &
         $ 0.69 {\scriptstyle \pm 0.01}$ &
         $ 0.33 {\scriptstyle \pm 0.00 }$ & 
         $ 0.37 {\scriptstyle \pm 0.02}$ \\
         
        GCN-dDGM$^{*}$-H&
         $ 0.89 {\scriptstyle \pm 0.01}$ &
         $ 0.66 {\scriptstyle \pm 0.01 }$ &
         $ 0.33 {\scriptstyle \pm 0.00 }$ & 
         $ 0.46 {\scriptstyle \pm 0.05 }$ \\
         
        GCN-dDGM$^{*}$-S&
         $ 0.86 {\scriptstyle \pm 0.03 }$ &
         $ 0.64 {\scriptstyle \pm 0.01}$ &
         $ 0.32 {\scriptstyle \pm 0.00 }$ & 
         $ 0.45  {\scriptstyle \pm 0.04 }$ \\ \midrule
         
        GCN-dDGM$^{*}$-HH&
         $ 0.91 {\scriptstyle \pm 0.01}$ &
         $  0.66 {\scriptstyle \pm 0.02}$ &
         $ 0.32 {\scriptstyle \pm 0.00}$ & 
         $ 0.37 {\scriptstyle \pm 0.01}$ \\
         
        GCN-dDGM$^{*}$-SS&
         $  0.85 {\scriptstyle \pm 0.02}$ &
         $ 0.51 {\scriptstyle \pm 0.01}$ &
         $ 0.27 {\scriptstyle \pm 0.00 }$ & 
         $ 0.31 {\scriptstyle \pm 0.01 }$ \\
         
         
        GCN-dDGM$^{*}$-EH&
         $ 0.90 {\scriptstyle \pm 0.01}$ &
         $ 0.65 {\scriptstyle \pm 0.01}$ &
         $ 0.32 {\scriptstyle \pm 0.00 }$ & 
         $ 0.43 {\scriptstyle \pm 0.03 }$ \\
         
       GCN-dDGM$^{*}$-ES&
         $ 0.91 {\scriptstyle \pm 0.00}$ &
         $ 0.63 {\scriptstyle \pm 0.02}$ &
         $ 0.27 {\scriptstyle \pm 0.02}$ & 
         $ 0.32 {\scriptstyle \pm 0.04 }$ \\
         
       GCN-dDGM$^{*}$-HS&
         $ 0.91 {\scriptstyle \pm 0.02 }$ &
         $ 0.67 {\scriptstyle \pm 0.02}$  &
         $ 0.33 {\scriptstyle \pm 0.00}$ & 
         $ 0.36 {\scriptstyle \pm 0.08 }$ \\

        GCN-dDGM$^{*}$-EHH&
         $ 0.90 {\scriptstyle \pm 0.05}$ &
         $ 0.59 {\scriptstyle \pm 0.04}$  &
         $  0.43 {\scriptstyle \pm 0.03}$ & 
         $ 0.55 {\scriptstyle \pm 0.03}$ \\
         
       GCN-dDGM$^{*}$-EHS&
         $ 0.91 {\scriptstyle \pm 0.03 }$ &
         $ 0.66 {\scriptstyle \pm 0.03 }$  &
         $ 0.32 {\scriptstyle \pm 0.01}$ & 
         $ 0.45 {\scriptstyle \pm 0.01 }$ \\

         
         
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:homophily_learning}
\end{table*}

==> tables/inductive_learning_model_summary.tex <==


\begin{table*}[htbp!]
    \centering
    \caption{Summary of model architectures for experiments for the QM9 and Alchemy datasets. These models incorporate a global mean pool layer since predictions are at the graph level, rather than at the node level as in all other datasets.
    }
    
\scalebox{0.83}{
    \begin{tabular}{lcc ccc}
    \toprule 
&  & &\multicolumn{3}{c}{Model}
    \\ \midrule
          &
& &
         \textbf{MLP} &  
         \textbf{GCN} & 
         \textbf{GCN-dDGM}
         \\ \midrule

         
         
         No. Layer parameters & BatchNorm & Activation & \multicolumn{3}{c}{Layer type}
         \\\midrule
          &  & & N/A & N/A & dDGM
          \\\hdashline
         (No. features, 20) & Yes (GraphNorm) & SiLU & Linear & Graph Conv & Graph Conv
          \\
          (20, 20) & Yes (GraphNorm) & SiLU & Linear & Graph Conv & Graph Conv
          \\ \hdashline
            &  & & \multicolumn{3}{c}{Global Mean Pool}
          \\ \hdashline
          
          (20, 20) & No & SiLU & Linear &  Linear & Linear
          \\ 
          (20, 20) & No & SiLU & Linear &  Linear & Linear
          \\ 
          (20, No. prediction targets) & No & - & Linear &  Linear & Linear
          \\ 
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:Summary of model inductive learning}
\end{table*}

==> tables/inductive_learning_results.tex <==


\begin{table*}[htbp!]
    \centering
    \caption{Results for the QM9 and Alchemy datasets using the dDGM module. 
    }
    
\scalebox{0.5}{
    \begin{tabular}{l cc}
    \toprule 
         &

         \textbf{QM9} &  
         \textbf{Alchemy} 

        
          
         
         \\ 


          
        No. graphs &  133,885
   
          & 119,487
          
\\
         Targets & 12
      
         & 12
          
         \\
         
         $k$ & 
    5
         &
         5
         \\
         \midrule
         
         Model &
         \multicolumn{2}{c}{R2 score ($\times 100$) $\pm$ Standard Deviation}
         
          
         
         \\ 

        
        \midrule

        GCN-dDGM$^{*}$-E&
         $ 96.23  {\scriptstyle \pm 1.55}$ &
         $ 96.11 {\scriptstyle \pm 1.43}$ \\
         
         
        
         GCN-dDGM$^{*}$-H&
         $ 97.50 {\scriptstyle \pm 1.04}$ &
         $ \thirdd{96.12 {\scriptstyle \pm 1.59}}$ \\
         
        GCN-dDGM$^{*}$-S&
         $ 96.52 {\scriptstyle \pm 2.30 }$ &
         $ 94.52 {\scriptstyle \pm 2.45}$ \\
         
        GCN-dDGM$^{*}$-HH&
         $ 96.53 {\scriptstyle \pm 2.03}$ &
         $ 95.06 {\scriptstyle \pm 1.59}$ \\
         
        GCN-dDGM$^{*}$-SS&
         $ 95.51 {\scriptstyle \pm 1.23}$ &
         $ 92.01 {\scriptstyle \pm 2.04 }$ \\
         
         
        GCN-dDGM$^{*}$-EH&
         $ \thirdd{97.79 {\scriptstyle \pm 1.24}}$ &
         $ \first{96.52 {\scriptstyle \pm 1.89}}$ \\
         
       GCN-dDGM$^{*}$-ES&
         $ 94.03 {\scriptstyle \pm 2.13}$ &
         $ 94.10 {\scriptstyle \pm 2.54 }$ \\
         
       GCN-dDGM$^{*}$-HS&
         $ 96.59 {\scriptstyle \pm 1.53 }$ &
         $ 96.00 {\scriptstyle \pm 1.01 }$ \\
         
       GCN-dDGM$^{*}$-EHS&
         $ 96.78 {\scriptstyle \pm 1.56 }$ &
         $ 96.03 {\scriptstyle \pm 2.59 }$ \\
         
         \midrule

        GCN-dDGM-E&
         $ \thirdd{97.79  {\scriptstyle \pm 1.34}}$ &
         $ 96.10 {\scriptstyle \pm 2.01}$ \\
         
         
        
         GCN-dDGM-H&
         $ 96.69 {\scriptstyle \pm 1.34}$ &
         $ 96.11 {\scriptstyle \pm 1.04}$ \\
         
        GCN-dDGM-S&
         $ 95.53 {\scriptstyle \pm 2.30 }$ &
         $ 91.98 {\scriptstyle \pm 2.40 }$ \\
         
        GCN-dDGM-HH&
         $ 96.78 {\scriptstyle \pm 1.05 }$ &
         $ \secondd{96.45{\scriptstyle \pm 2.54}}$ \\
         
        GCN-dDGM-SS&
         $ 96.45 {\scriptstyle \pm 2.32 }$ &
         $ 93.67 {\scriptstyle \pm 3.01}$ \\
         
         
        GCN-dDGM-EH&
         $ \first{98.00 {\scriptstyle \pm 1.34 }}$ &
         $ 96.04 {\scriptstyle \pm 1.45 }$ \\
         
       GCN-dDGM-ES&
         $ 96.52 {\scriptstyle \pm 1.54 }$ &
         $ 95.02 {\scriptstyle \pm 1.23 }$ \\
         
       GCN-dDGM-HS&
         $ 96.51 {\scriptstyle \pm 1.23 }$ &
         $ 95.39 {\scriptstyle \pm 1.01 }$ \\
         
       GCN-dDGM-EHS&
         $ \secondd{97.99 {\scriptstyle \pm 1.02 }}$ &
         $ 96.02 {\scriptstyle \pm 2.10 }$ \\
         
         \midrule

         MLP$^{*}$ &
         $ 82.20 {\scriptstyle \pm 3.80}$ &
         $ 76.56 {\scriptstyle \pm 1.50}$  \\ 
         
         GCN &
         $ 94.35 {\scriptstyle \pm 1.30}$ &
         $ 95.15 {\scriptstyle \pm 1.43}$ \\

         
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:inductive_learning_results}
\end{table*}

==> tables/main_results.tex <==

\newcommand{\first}[1]{\mathbf{\textcolor{red}{#1}}}
\newcommand{\secondd}[1]{\mathbf{\textcolor{blue}{#1}}}
\newcommand{\thirdd}[1]{\mathbf{\textcolor{violet}{#1}}}

\begin{table*}[htbp!]
    \centering
    \caption{Results for  heterophilic and homophilic datasets combining GCN diffusion layers with the latent graph inference system. We display results using model spaces as well as product manifolds to construct the latent graphs. The \textbf{\textcolor{red}{First}}, \textbf{\textcolor{blue}{Second}} and \textbf{\textcolor{violet}{Third}} best models for each dataset are highlighted in each table. $k$ denotes the number of connections per node when implementing the Gumbel Top-k sampling algorithm. Additional $k$ values are tested in Appendix~\ref{appendix:Homophilic Graph Datasets Extended Results}}
    
\scalebox{0.46}{
    \begin{tabular}{l cccc l ccccc}
    \toprule 
         &

         \multicolumn{4}{c}{HETEROPHILIC DATASETS}
         &

         & \multicolumn{4}{c}{HOMOPHILIC DATASETS}
         \\
         
    \toprule 
         &

         \textbf{Texas} &  
         \textbf{Wisconsin} & 
         \textbf{Squirrel} &
         \textbf{Chameleon} &  &
         \textbf{Cora} &
         \textbf{CiteSeer} &
         \textbf{PubMed} &
         \textbf{Physics} &
         \textbf{CS}
         \\
         
         Homophily level &
         0.11 &
         0.21 &
         0.22 &
         0.23 &
         Homophily level&
         0.81 &
         0.74 &
         0.80 &
         0.93&
         0.80
         
          \\ 
         
         Nodes &
    
         183 &
         251 &
         5,201 &
           2,277&
         Nodes&
         2,708 &
         3,327 &
         18,717 &
          34,493 &
          18,333
          \\
          
        Features &
   
         1,703 &
         1,703 &
         2,089 &
          2,325&
         Features&
         1,433 &
         3,703 &
         500 &
          8,415 &
          6,805
          \\
         
         Edges &
        
        295 &
         466 &
         198,498 &
         31,421 &
         Edges&
          5,278 &
         4,676 &
         44,327 &
         247,962 &
         81,894
          \\
         
         Classes &
      
        5 &
         5 &
         5 &
         5&
         Classes&
         7 &
         6 &
         3 &
         5 &
         15\\
         
         Average Degree & 
      
        3.22 &
         3.71 &
         76.33 &
         27.60&
         Average Degree&
         3.9 &
         2.77 &
         4.5 &
         14.38 &
         8.93\\
         
         
         \midrule
         
         Model &
         \multicolumn{4}{c}{Accuracy $(\%)$ $\pm$ Standard Deviation} &
         Model &
         \multicolumn{4}{c}{Accuracy $(\%)$ $\pm$ Standard Deviation}
\\
         $k$ & 
    
        2 &
         10 &
         3 &
         5&
          $k$ &7
         & 7
         & 7
         & 5
         & 7
         
          
         
          
         
         \\ 

        
        \midrule
        GCN-dDGM$^{*}$-E&
         $ \thirdd{80.00 {\scriptstyle \pm 8.31 }}$ &
         $ \thirdd{88.00 {\scriptstyle \pm 5.65}}$ &
         $ 34.35 {\scriptstyle \pm 2.34 }$ & 
         $ \first{48.90 {\scriptstyle \pm 3.61}}$ &
         GCN-dDGM-E&
         $82.11 {\scriptstyle \pm 4.24}$
         & $72.35 {\scriptstyle \pm 1.92}$
         & $\thirdd{87.69 {\scriptstyle \pm 0.67}}$
         & $95.96 {\scriptstyle \pm 0.40}$
         & $87.17 {\scriptstyle \pm 3.82}$\\
         
        GCN-dDGM$^{*}$-H&
         $ 79.44 {\scriptstyle \pm 7.88}$ &
         $ \secondd{89.03 {\scriptstyle \pm 1.89 }}$ &
         $ \first{35.00 {\scriptstyle \pm 2.35}}$ & 
         $ 48.28 {\scriptstyle \pm 4.11 }$&
         GCN-dDGM-H&
         $ \secondd{84.68 {\scriptstyle \pm 3.31}}$
         & $70.43 {\scriptstyle \pm 4.95}$
         & $\secondd{87.74 {\scriptstyle \pm 0.72}}$
         & $\secondd{96.06 {\scriptstyle \pm 0.42}}$
         & $88.78 {\scriptstyle \pm 2.24}$\\
         
        GCN-dDGM$^{*}$-S&
         $ 73.88 {\scriptstyle \pm 9.95}$ &
         $ 85.33 {\scriptstyle \pm 4.98}$ &
         $ 33.12 {\scriptstyle \pm 2.22}$ & 
         $ \secondd{48.63{\scriptstyle \pm 3.12 }}$&
         GCN-dDGM-S&
         $80.44 {\scriptstyle \pm 5.26}$
         & $\secondd{72.89 {\scriptstyle \pm 2.00}}$
         & $87.13 {\scriptstyle \pm 0.66}$
         & $95.91 {\scriptstyle \pm 0.41}$
         & $84.16 {\scriptstyle \pm 2.78}$\\\midrule

         
         Model &
         \multicolumn{4}{c}{Accuracy $(\%)$ $\pm$ Standard Deviation} &
         Model &
         \multicolumn{4}{c}{Accuracy $(\%)$ $\pm$ Standard Deviation}
\\
         $k$ & 
    
        2 &
         10 &
         3 &
         5&
          $k$ &5
         & 3
         & 10
         & 10
         & 3
         
          
         
          
         
         \\ 

        
        \midrule
         
        GCN-dDGM$^{*}$-HH&
         $ 78.89 {\scriptstyle \pm 8.53 }$ &
         $ \thirdd{88.00 {\scriptstyle \pm 3.26 }}$ &
         $ \thirdd{34.38 {\scriptstyle \pm 1.07}}$ & 
         $ \thirdd{48.33 {\scriptstyle \pm 4.14}}$&
         GCN-dDGM-HH&
         $76.09 {\scriptstyle \pm 7.11}$
         & $71.27 {\scriptstyle \pm 2.09}$
         & $87.50 {\scriptstyle \pm 0.91}$
         & $94.73 {\scriptstyle \pm 2.83}$
         & $82.91 {\scriptstyle \pm 3.00}$\\
         
        GCN-dDGM$^{*}$-SS&
         $ 73.89 {\scriptstyle \pm 8.62 }$ &
         $  74.66 {\scriptstyle \pm 18.85  }$ &
         $ 34.06 {\scriptstyle \pm 2.20 }$ & 
         $ 48.28 {\scriptstyle \pm 3.07}$&
         GCN-dDGM-SS&
         $65.96 {\scriptstyle \pm 9.46}$
         & $59.16 {\scriptstyle \pm 5.96}$
         & $\first{87.82 {\scriptstyle \pm 0.59}}$
         & $90.72 {\scriptstyle \pm 5.26}$
         & $59.31 {\scriptstyle \pm 7.18}$\\
         
         
        GCN-dDGM$^{*}$-EH&
         $ \first{81.67 {\scriptstyle \pm 7.05}}$ &
         $ 86.67 {\scriptstyle \pm 3.77}$ &
         $ 34.37 {\scriptstyle \pm 1.72}$ & 
         $ 47.58 {\scriptstyle \pm 3.85}$&
         GCN-dDGM-EH&
         $82.32 {\scriptstyle \pm 4.71}$
         & $\secondd{72.89 {\scriptstyle \pm 1.64}}$
         & $87.41 {\scriptstyle \pm 0.80}$
         & $\thirdd{96.03 {\scriptstyle \pm 0.37}}$
         & $\secondd{91.37 {\scriptstyle \pm 1.28}}$\\
         
       GCN-dDGM$^{*}$-ES&
         $ \secondd{81.11 {\scriptstyle \pm 10.30}}$ &
         $ 76.00 {\scriptstyle \pm 11.31 }$ &
         $ 33.38 {\scriptstyle \pm 1.86}$ & 
         $ 47.49 {\scriptstyle \pm 3.60}$&
         GCN-dDGM-ES&
         $81.44 {\scriptstyle \pm 5.80}$
         & $71.87 {\scriptstyle \pm 3.20}$
         & $87.50 {\scriptstyle \pm 0.65}$
         & $95.41 {\scriptstyle \pm 1.73}$
         & $\thirdd{90.87 {\scriptstyle \pm 0.82}}$\\
         
       GCN-dDGM$^{*}$-HS&
         $ \secondd{81.11 {\scriptstyle \pm 9.69}}$ &
         $ 86.67 {\scriptstyle \pm 1.89 }$ &
         $ \secondd{34.65 {\scriptstyle \pm 2.45}}$ & 
         $ 47.84 {\scriptstyle \pm 2.67}$&
         GCN-dDGM-HS&
         $82.59 {\scriptstyle \pm 4.50}$
         & $\thirdd{72.77 {\scriptstyle \pm 2.76}}$
         & $85.89 {\scriptstyle \pm 4.29}$
         & $95.84 {\scriptstyle \pm 0.29}$
         & $89.43 {\scriptstyle \pm 2.37}$\\

         GCN-dDGM$^{*}$-EHH&
         $ \secondd{81.11 {\scriptstyle \pm 5.09}}$
          & $77.60 {\scriptstyle \pm 8.62}$
         &$33.19  {\scriptstyle \pm 1.92}$
         & $44.27 {\scriptstyle \pm 2.96}$
         &
         GCN-dDGM-EHH&
         $ \first{86.63 {\scriptstyle \pm 3.25}}$
         & $\first{75.42 {\scriptstyle \pm 2.39}}$
         & $39.93 {\scriptstyle \pm 1.35}$
         & $95.63 {\scriptstyle \pm 1.36}$
         & $\first{92.86 {\scriptstyle \pm 0.96}}$\\
         
       GCN-dDGM$^{*}$-EHS&
         $ 79.44 {\scriptstyle \pm 6.11}$ &
         $ \first{89.33 {\scriptstyle \pm 1.89 }}$ &
         $ 34.17 {\scriptstyle \pm 2.23}$ & 
         $ 47.58 {\scriptstyle \pm 4.54}$ &
         GCN-dDGM-EHS&
         $ \thirdd{83.58 {\scriptstyle \pm 4.39}}$
         & $69.98 {\scriptstyle \pm 2.70}$
         & $87.05 {\scriptstyle \pm 1.38}$
         & $\first{96.21 {\scriptstyle \pm 0.44}}$
         & $89.93 {\scriptstyle \pm 3.86}$\\
         
         
         
         \midrule
         
         MLP$^{*}$ &
         $ 77.78 {\scriptstyle \pm 10.24}$ &
         $ 85.33 {\scriptstyle \pm 4.99}$ &
         $ 30.44 {\scriptstyle \pm 2.55}$ & 
         $ 40.35 {\scriptstyle \pm 3.37}$ &
         MLP$^{*}$
         &
         $ 58.92 {\scriptstyle \pm 3.28}$ &
         $ 59.48 {\scriptstyle \pm 2.14}$&
         $ 85.75{\scriptstyle \pm 1.02}$&
         $ 94.91 {\scriptstyle \pm 0.30}$&  
         $  87.80 {\scriptstyle \pm 1.54 }$
         \\

         GCN &
         $ 41.66 {\scriptstyle \pm 11.72}$ &
         $ 47.20 {\scriptstyle \pm 9.76}$ &
         $ 24.19 {\scriptstyle \pm 2.56}$ & 
         $ 32.56 {\scriptstyle \pm 3.53}$&
         GCN
         &$ 83.11 {\scriptstyle \pm 2.29}$ &
         $ 69.97 {\scriptstyle \pm 2.06}$ &
         $ 85.75 {\scriptstyle \pm 1.01}$ & 
         $ 95.51 {\scriptstyle \pm 0.34}$ &
         $ 87.28 {\scriptstyle \pm 1.54 }$\\ 

         
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:main_results}
\end{table*}

==> tables/more_complex_manifolds.tex <==


\begin{table*}[hbpt!]
    \centering
    \caption{Results using more complex product manifolds for the CS dataset. We multiply up to five model spaces to generate the product manifolds.
    }
    
\scalebox{0.65}{
    \begin{tabular}{l cc}
    \toprule 
         &
         &

         \textbf{CS}
         \\
         \midrule
         
         Model & $k$ &
         \multicolumn{1}{c}{Accuracy $(\%)$ $\pm$ Standard Deviation}
         
         \\
          \midrule

                   GCN-dDGM-E & 3&
         $ 85.98 {\scriptstyle \pm 2.59 }$\\

                  GCN-dDGM-H & 3&
         $ 85.95 {\scriptstyle \pm 2.58}$\\

                  GCN-dDGM-S & 3&
         $ 76.76 {\scriptstyle \pm 4.65}$\\ \midrule

                  GCN-dDGM-EH & 3&
         $ 91.37 {\scriptstyle \pm 1.28 }$\\

                  GCN-dDGM-ES & 3&
         $ 90.87 {\scriptstyle \pm 0.82 }$\\

                  GCN-dDGM-HS & 3&
         $ 89.43 {\scriptstyle \pm 2.37}$\\

                  GCN-dDGM-EHH & 3&
         $ 92.86 {\scriptstyle \pm 0.96 }$\\

                  GCN-dDGM-EHS & 3&
         $ 89.93 {\scriptstyle \pm 3.86 }$\\

                  GCN-dDGM-EHHH & 3&
         $ 92.86 {\scriptstyle \pm 1.04}$\\

                  GCN-dDGM-EHHS & 3&
         $ 92.70 {\scriptstyle \pm 0.66 }$\\

                  GCN-dDGM-EHHSH & 3&
         $ \secondd{92.96 {\scriptstyle \pm 0.46}}$\\
         GCN-dDGM-EHHSS & 3&
         $ 91.51{\scriptstyle \pm 2.51 }$\\
         
         \midrule

         
         GCN-dDGM-E & 5&
         $ 87.88 {\scriptstyle \pm 2.55}$\\

                  GCN-dDGM-H & 5&
         $ 87.65 {\scriptstyle \pm 2.56}$\\

                  GCN-dDGM-S & 5&
         $ 80.73 {\scriptstyle \pm 4.62 }$\\ \midrule

                  GCN-dDGM-EH & 5&
         $ 91.11 {\scriptstyle \pm 1.57}$\\

                  GCN-dDGM-ES & 5&
         $ 89.31 {\scriptstyle \pm 2.31}$\\

                  GCN-dDGM-HS & 5&
         $ 90.98 {\scriptstyle \pm 1.00}$\\

                  GCN-dDGM-EHH & 5&
         $92.30 {\scriptstyle \pm 1.05}$\\

                  GCN-dDGM-EHS & 5&
         $92.06 {\scriptstyle \pm 0.83}$\\

                  GCN-dDGM-EHHH & 5&
         $ 92.63 {\scriptstyle \pm 0.63}$\\

                  GCN-dDGM-EHHS & 5&
         $ 92.82 {\scriptstyle \pm 1.34 }$\\

                  GCN-dDGM-EHHSH & 5&
         $ \thirdd{92.91 {\scriptstyle \pm 0.66 }}$\\

                  GCN-dDGM-EHHSS & 5&
         $ \first{93.10 {\scriptstyle \pm 0.74 }}$\\

         


         \midrule
         GCN & N/A &
         $ 87.28 {\scriptstyle \pm 1.54 }$\\ 
         

         
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:more_complex}
\end{table*}

==> tables/no_layers_asterisk.tex <==


\begin{table*}[htbp!]
    \centering
    \caption{Results for Cora, CiteSeer, and PubMed using more than one dDGM$^{*}$ (taking a pointcloud as input) latent graph inference module.}
    
\scalebox{0.65}{
    \begin{tabular}{l clccc}
    \toprule 
         &
         &
         &
         \textbf{Cora} &  
         \textbf{CiteSeer} & 
         \textbf{PubMed} 

          
\\
         \midrule
         
         Model & $k$ & \multicolumn{1}{c}{Layers} &
         \multicolumn{3}{c}{Accuracy $(\%)$ $\pm$ Standard Deviation}
         
         \\

        
        \midrule

         
         GCN-dDGM$^{*}$-E & 3&
         dDGM$^{*}$/GCN/GCN/GCN &
         $ 62.48 {\scriptstyle \pm 3.24}$ &
         $ 62.47 {\scriptstyle \pm 3.20}$ &
         $ 83.89 {\scriptstyle \pm 0.70}$ \\

         GCN-dDGM$^{*}$-E & 3&
         dDGM$^{*}$/GCN/dDGM$^{*}$/GCN/GCN &
         $ 54.22 {\scriptstyle \pm 3.79 }$ &
         $ 59.76 {\scriptstyle \pm 2.18 }$ &
         $ 85.74 {\scriptstyle \pm 2.06}$ \\

         % GCN-dDGM-E$^{*}$ & 3&
         % dDGM/GCN/dDGM/GCN/dDGM/GCN &
         % $  {\scriptstyle \pm }$ &
         % $ {\scriptstyle \pm }$ &
         % $  {\scriptstyle \pm }$ \\
         
         \midrule

         GCN-dDGM$^{*}$-EH & 3&
         dDGM$^{*}$/GCN/GCN/GCN &
         $ 61.07 {\scriptstyle \pm 10.18}$ &
         $ \first{65.13 {\scriptstyle \pm 2.19}}$ &
         $ 86.67 {\scriptstyle \pm 0.69}$ \\

         GCN-dDGM$^{*}$-EH & 3&
         dDGM$^{*}$/GCN/dDGM$^{*}$/GCN/GCN &
         $ 51.96 {\scriptstyle \pm 4.53}$ &
         $ 55.36 {\scriptstyle \pm 5.35}$ &
         $ 86.19 {\scriptstyle \pm 1.10}$ \\

         % GCN-dDGM-EH$^{*}$ & 3&
         % dDGM/GCN/dDGM/GCN/dDGM/GCN &
         % $  {\scriptstyle \pm }$ &
         % $ {\scriptstyle \pm }$ &
         % $  {\scriptstyle \pm }$ \\ 
         
         \midrule

         GCN-dDGM$^{*}$-EHS & 3&
         dDGM$^{*}$/GCN/GCN/GCN &
         $ \first{66.87 {\scriptstyle \pm 3.27}}$ &
         $ \thirdd{63.80 {\scriptstyle \pm 2.94}}$ &
         $ \first{87.03 {\scriptstyle \pm 0.70}}$ \\

         GCN-dDGM$^{*}$-EHS & 3&
         dDGM$^{*}$/GCN/dDGM$^{*}$/GCN/GCN &
         $ 50.66 {\scriptstyle \pm 4.26}$ &
         $ 51.66 {\scriptstyle \pm 3.24}$ &
         $ 86.32 {\scriptstyle \pm 0.70}$ \\

         % GCN-dDGM-EHS$^{*}$ & 3&
         % dDGM/GCN/dDGM/GCN/dDGM/GCN &
         % $  {\scriptstyle \pm }$ &
         % $ {\scriptstyle \pm }$ &
         % $  {\scriptstyle \pm }$ \\ 
         
         \midrule

         
         GCN-dDGM$^{*}$-E & 5&
         dDGM$^{*}$/GCN/GCN/GCN &
         $ 60.63 {\scriptstyle \pm 3.01}$ &
         $ 63.28 {\scriptstyle \pm 3.35 }$ &
         $ 86.82 {\scriptstyle \pm 0.69}$ \\

         GCN-dDGM$^{*}$-E & 5&
         dDGM$^{*}$/GCN/dDGM$^{*}$/GCN/GCN &
         $ 52.15 {\scriptstyle \pm 4.21}$ &
         $ 54.46 {\scriptstyle \pm 3.19}$ &
         $  79.04 {\scriptstyle \pm 4.45 }$ \\

         % GCN-dDGM-E$^{*}$ & 5&
         % dDGM/GCN/dDGM/GCN/dDGM/GCN &
         % $  {\scriptstyle \pm }$ &
         % $ {\scriptstyle \pm }$ &
         % $  {\scriptstyle \pm }$ \\ 
         
         \midrule

         GCN-dDGM$^{*}$-EH & 5&
         dDGM$^{*}$/GCN/GCN/GCN &
         $ \thirdd{63.67 {\scriptstyle \pm 6.48}}$ &
         $ 61.59 {\scriptstyle \pm 12.28}$ &
         $ \thirdd{86.90 {\scriptstyle \pm 1.16}}$ \\

         GCN-dDGM$^{*}$-EH & 5&
         dDGM$^{*}$/GCN/dDGM$^{*}$/GCN/GCN &
         $ 45.30 {\scriptstyle \pm 3.06}$ &
         $ 51.69 {\scriptstyle \pm 4.33 }$ &
         $ 82.02 {\scriptstyle \pm 5.42}$ \\

         % GCN-dDGM-EH$^{*}$ & 5&
         % dDGM/GCN/dDGM/GCN/dDGM/GCN &
         % $  {\scriptstyle \pm }$ &
         % $ {\scriptstyle \pm }$ &
         % $  {\scriptstyle \pm }$ \\ 
         
         \midrule

         GCN-dDGM$^{*}$-EHS & 5&
         dDGM$^{*}$/GCN/GCN/GCN &
         $ \secondd{64.82 {\scriptstyle \pm 3.68}}$ &
         $ \secondd{64.62 {\scriptstyle \pm 3.35}}$ &
         $ 86.85 {\scriptstyle \pm 0.97 }$ \\

         GCN-dDGM$^{*}$-EHS & 5&
         dDGM$^{*}$/GCN/dDGM$^{*}$/GCN/GCN &
         $ 45.07 {\scriptstyle \pm 4.21 }$ &
         $ 45.42 {\scriptstyle \pm 3.00 }$ &
         $ \secondd{86.92 {\scriptstyle \pm 0.83 }}$ \\

         % GCN-dDGM-EHS$^{*}$ & 5&
         % dDGM/GCN/dDGM/GCN/dDGM/GCN &
         % $  {\scriptstyle \pm }$ &
         % $ {\scriptstyle \pm }$ &
         % $  {\scriptstyle \pm }$ \\ 
         
         \midrule

        
         MLP$^{*}$ & N/A &
         Linear/Linear/Linear&
         $ 58.92 {\scriptstyle \pm 3.28}$ &
         $ 59.48 {\scriptstyle \pm 2.14}$ &
         $ 85.75{\scriptstyle \pm 1.02}$ \\ 

         
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:no_layers_asterick}
\end{table*}

==> tables/no_layers_no_asterisk.tex <==


\begin{table*}[htbp!]
    \centering
    \caption{Results for Cora, CiteSeer, and PubMed using more than one dDGM (leveraging the original graph connectivity structure) latent graph inference module.
    }
    
\scalebox{0.65}{
    \begin{tabular}{l clccc}
    \toprule 
         &
         &
         &
         \textbf{Cora} &  
         \textbf{CiteSeer} & 
         \textbf{PubMed} 
         
         \\ 
         \midrule
         
         Model & $k$ & \multicolumn{1}{c}{Layers} &
         \multicolumn{3}{c}{Accuracy $(\%)$ $\pm$ Standard Deviation}
         
         \\

        
        \midrule

         
         GCN-dDGM-E & 3&
         dDGM/GCN/GCN/GCN &
         $ 80.44 {\scriptstyle \pm 4.60 }$ &
         $ 70.18 {\scriptstyle \pm 1.46}$ &
         $  87.45 {\scriptstyle \pm 0.72}$ \\

         GCN-dDGM-E & 3&
         dDGM/GCN/dDGM/GCN/GCN &
         $ 70.44 {\scriptstyle \pm 5.81 }$ &
         $ 69.85 {\scriptstyle \pm 4.22}$ &
         $ 86.67 {\scriptstyle \pm 0.48}$ \\

         % GCN-dDGM-E & 3&
         % dDGM/GCN/dDGM/GCN/dDGM/GCN &
         % $  {\scriptstyle \pm }$ &
         % $ {\scriptstyle \pm }$ &
         % $  {\scriptstyle \pm }$ \\ 
         
         \midrule

         GCN-dDGM-EH & 3&
         dDGM/GCN/GCN/GCN &
         $ \secondd{83.65 {\scriptstyle \pm 5.25}}$ &
         $ \thirdd{72.89 {\scriptstyle \pm 1.64}}$ &
         $ \secondd{87.62 {\scriptstyle \pm 0.64}}$ \\

         GCN-dDGM-EH & 3&
         dDGM/GCN/dDGM/GCN/GCN &
         $ 77.30 {\scriptstyle \pm 7.30}$ &
         $ 72.32 {\scriptstyle \pm 2.09}$ &
         $ 87.02 {\scriptstyle \pm 0.79}$ \\

         % GCN-dDGM-EH & 3&
         % dDGM/GCN/dDGM/GCN/dDGM/GCN &
         % $  {\scriptstyle \pm }$ &
         % $ {\scriptstyle \pm }$ &
         % $  {\scriptstyle \pm }$ \\ 
         
         \midrule

         GCN-dDGM-EHS & 3&
         dDGM/GCN/GCN/GCN &
         $ \first{84.70 {\scriptstyle \pm 2.96}}$ &
         $ 69.98 {\scriptstyle \pm 2.70}$ &
         $ 87.35 {\scriptstyle \pm 0.90}$ \\

         GCN-dDGM-EHS & 3&
         dDGM/GCN/dDGM/GCN/GCN &
         $ 79.07 {\scriptstyle \pm 4.35}$ &
         $ 71.99 {\scriptstyle \pm 1.94}$ &
         $ 86.93 {\scriptstyle \pm 0.71}$ \\

         % GCN-dDGM-EHS & 3&
         % dDGM/GCN/dDGM/GCN/dDGM/GCN &
         % $  {\scriptstyle \pm }$ &
         % $ {\scriptstyle \pm }$ &
         % $  {\scriptstyle \pm }$ \\ 
         
         \midrule

         
         GCN-dDGM-E & 5&
         dDGM/GCN/GCN/GCN &
         $ 82.74 {\scriptstyle \pm 4.42}$ &
         $ 71.78 {\scriptstyle \pm 1.50 }$ &
         $ \thirdd{87.60 {\scriptstyle \pm 0.69}}$ \\

         GCN-dDGM-E & 5&
         dDGM/GCN/dDGM/GCN/GCN &
         $ 72.70 {\scriptstyle \pm 6.03 }$ &
         $ 68.25 {\scriptstyle \pm 4.57}$ &
         $ 86.59 {\scriptstyle \pm 0.87}$ \\

         % GCN-dDGM-E & 5&
         % dDGM/GCN/dDGM/GCN/dDGM/GCN &
         % $  {\scriptstyle \pm }$ &
         % $ {\scriptstyle \pm }$ &
         % $  {\scriptstyle \pm }$ \\ 
         
         \midrule

         GCN-dDGM-EH & 5&
         dDGM/GCN/GCN/GCN &
         $ 82.32 {\scriptstyle \pm 4.71}$ &
         $ \secondd{73.56 {\scriptstyle \pm 2.75 }}$ &
         $ \first{87.67 {\scriptstyle \pm 0.76}}$ \\

         GCN-dDGM-EH & 5&
         dDGM/GCN/dDGM/GCN/GCN &
         $ 76.04 {\scriptstyle \pm 4.23}$ &
         $ 72.11 {\scriptstyle \pm 2.33 }$ &
         $ 86.49 {\scriptstyle \pm 0.73}$ \\

         % GCN-dDGM-EH & 5&
         % dDGM/GCN/dDGM/GCN/dDGM/GCN &
         % $  {\scriptstyle \pm }$ &
         % $ {\scriptstyle \pm }$ &
         % $  {\scriptstyle \pm }$ \\ 
         
         \midrule

         GCN-dDGM-EHS & 5&
         dDGM/GCN/GCN/GCN &
         $ \thirdd{83.58 {\scriptstyle \pm 4.39 }}$ &
         $ \first{74.00 {\scriptstyle \pm 1.68}}$ &
         $ 87.12 {\scriptstyle \pm 0.72}$ \\

         GCN-dDGM-EHS & 5&
         dDGM/GCN/dDGM/GCN/GCN &
         $ 76.67 {\scriptstyle \pm 5.55}$ &
         $ 70.42 {\scriptstyle \pm 1.66 }$ &
         $ 82.57  {\scriptstyle \pm 0.81}$ \\

         % GCN-dDGM-EHS & 5&
         % dDGM/GCN/dDGM/GCN/dDGM/GCN &
         % $  {\scriptstyle \pm }$ &
         % $ {\scriptstyle \pm }$ &
         % $  {\scriptstyle \pm }$ \\ 
         
         \midrule

        
         GCN & N/A &
         GCN/GCN/GCN&
         $ 83.11 {\scriptstyle \pm 2.29}$ &
         $ 69.97 {\scriptstyle \pm 2.06}$ &
         $ 85.75 {\scriptstyle \pm 1.01}$ \\ 

         
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:no_layers_no_asterick}
\end{table*}

==> tables/ogb_products_model_summary.tex <==


\begin{table*}[htbp!]
    \centering
    \caption{Summary of model architectures for experiments for the OGB-Products dataset using GATv2 diffusion layers, with $k=3$ for the dDGM module.
    }
    
\scalebox{0.78}{
    \begin{tabular}{lcc ccc}
    \toprule 
&  & &\multicolumn{3}{c}{Model}
    \\ \midrule
          &
& &
         \textbf{MLP} &  
         \textbf{GATv2} & 
         \textbf{GATv2-dDGM}
         \\ \midrule

         
         
         No. Layer parameters & BatchNorm & Activation & \multicolumn{3}{c}{Layer type}
         \\\midrule
          &  & & N/A & N/A & dDGM ($k=3$)
          \\\hdashline
         ($\textrm{No. features} = 100$, 100) & No & SiLU & Linear & Graph Attention v2 & Graph Attention v2
          \\
          (100, 100) & No & SiLU & Linear & Graph Attention v2 & Graph Attention v2
          \\
          (100, 47) & No & SiLU & Linear & Graph Attention v2 & Graph Attention v2
          \\
          (47, $\textrm{No. classes} = 47$) & No & - & Linear &  Linear & Linear
          \\ 
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:Summary of model architecture products}
\end{table*}

==> tables/products.tex <==


\begin{table*}[htbp!]
    \centering
    \caption{Results for OGB-Products dataset using GATv2 diffusion layers and different latent graph inference modules.
    }
    
\scalebox{0.65}{
    \begin{tabular}{lcc}
    \toprule 
         &  &
         \textbf{OGB-Products}

         
          \\ 
         
         Nodes & &
        
          2,449,029	
          \\

    
         
         
          
        Features & &
        
100
          
          \\

          Edges & &

          61,859,140\\
         
         
         Classes & &
        
         47 \\

         
        
         \midrule
         
         Model & $k$ &
         \multicolumn{1}{c}{Accuracy $(\%)$ $\pm$ Standard Deviation}
         
         \\
          \midrule

        GATv2-dDGM-E & 3 &
         $\first{66.59 {\scriptstyle \pm 0.30  }}$\\

         GATv2-dDGM-H & 3 &
         $ 62.22{\scriptstyle \pm 0.25}$\\

        GATv2-dDGM-EH & 3 &
         $65.51 {\scriptstyle \pm 0.30 }$\\
         
         \midrule

        GATv2-dDGM-E & 5 &
         $ \secondd{66.25 {\scriptstyle \pm  0.71}}$\\

         GATv2-dDGM-H & 5 &
         $ 63.95 {\scriptstyle \pm 0.42}$\\

        GATv2-dDGM-EH & 5 &
         $65.62 {\scriptstyle \pm  0.20}$\\
         
         \midrule
         
         MLP$^{*}$ & N/A &
         $ \thirdd{66.05 {\scriptstyle \pm 0.20} }$ \\ 

         GATv2 & N/A &
         $ 62.02 {\scriptstyle \pm 2.60 }$ \\ 
         

         
         \bottomrule
         
        \end{tabular}}
    
    \label{tab:products}
\end{table*}

==> tables/real_world_applications.tex <==



\scalebox{0.5}{
    \begin{tabular}{lcc}
    \toprule 
         &
         \textbf{TadPole}

         &
         \textbf{Aerothermodynamics}

         
          \\ 
         
         Nodes &
          564 & 1,456
          \\
          
        Features &
          30 & 1
          \\
         
         
         Classes &
         3 & 4\\
        
         
        
         \midrule
         
         Model &
         \multicolumn{2}{c}{Accuracy $(\%)$ $\pm$ Standard Deviation}
         
         \\
          \midrule

         GAT-dDGM$^{*}$-E & 
         $ \thirdd{90.36 {\scriptstyle \pm 3.21}}$& $ 89.20 {\scriptstyle \pm 1.81}$\\

         GAT-dDGM$^{*}$-H & 
         $ 88.75 {\scriptstyle \pm 3.91 }$& $ 86.36 {\scriptstyle \pm 2.99}$\\

         GAT-dDGM$^{*}$-S & 
         $ \secondd{90.89 {\scriptstyle \pm 4.55 }}$&$ 86.21 {\scriptstyle \pm 5.37 }$\\

         GAT-dDGM$^{*}$-HH & 
         $  89.68 {\scriptstyle \pm 5.70 }$&$ 77.47 {\scriptstyle \pm 13.81 }$\\

         GAT-dDGM$^{*}$-SS & 
         $ 89.82 {\scriptstyle \pm 4.79}$&$  71.26 {\scriptstyle \pm 14.40  }$\\


         
         GAT-dDGM$^{*}$-EH & 
         $ \thirdd{90.36 {\scriptstyle \pm 4.16 }}$ &$\thirdd{89.90 {\scriptstyle \pm 0.55 }}$\\
         
         
         GAT-dDGM$^{*}$-ES & 
         $ 89.46 {\scriptstyle \pm  5.56 }$& $ \secondd{90.34 {\scriptstyle \pm 3.90 }}$\\
         
         GAT-dDGM$^{*}$-HS &
         $ 86.43 {\scriptstyle \pm 5.82}$& $  88.73 {\scriptstyle \pm 4.72  }$\\

         GAT-dDGM$^{*}$-EHH & 
         $ 87.68 {\scriptstyle \pm 9.95}$ &$  \first{91.72 {\scriptstyle \pm 0.98}}$\\
         
         GAT-dDGM$^{*}$-EHS & 
         $ \first{92.68 {\scriptstyle \pm 3.52}}$&$  88.74 {\scriptstyle \pm 3.39 }$\\
         
         \midrule
         MLP$^{*}$ & $87.68 {\scriptstyle \pm 3.52}$& $ 81.03 {\scriptstyle \pm 8.56}$ \\ 
         

         
         \bottomrule
         
        \end{tabular}}


==> tables/runtime.tex <==
\begin{table*}[htbp!]
    \centering
    \caption{Results for runtime speedup quantification using symbolic as compared to dense matrices. These results are for the GCN-dDGM-E model using $k=3$ and training for 100 epochs using NVIDIA P100 GPU.
    }
    
\scalebox{0.65}{
    \begin{tabular}{ccclc}
    \toprule 
         Model &
         No. dDGMs &
         Matrix &
         Dataset &
         Runtime (s) $\pm$ Standard Deviation
         \\ \midrule
        \multirow{12}{*}{GCN-dDGM-E} &
        1 & 
        Dense&
        Cora & $2.98 {\scriptstyle\pm 0.01}$
        
         
         \\
          &
         1 & 
        Symbolic&
        Cora & $2.64 {\scriptstyle\pm 0.01}$
        
         
         \\
          &
         1 & 
        Dense&
        CiteSeer & $3.50{\scriptstyle \pm 0.02}$
        
         
         \\
          &
         1 & 
        Symbolic&
        CiteSeer &  $2.73 {\scriptstyle\pm 0.02}$
        
         
         \\
         &
         2 & 
        Dense&
        Cora & $4.87{\scriptstyle \pm 0.19}$
        
         
         \\
        &
         2 & 
        Symbolic&
        Cora & $4.03  {\scriptstyle\pm 0.03}$
        
         
         \\
        &
         2 & 
        Dense&
        CiteSeer & $6.16 {\scriptstyle\pm 0.58}$
        
         
         \\
         &
         2 & 
        Symbolic&
        CiteSeer & $4.13 {\scriptstyle\pm 0.02}$
        
         
         \\
         &
         3 & 
        Dense&
        Cora & $6.53 {\scriptstyle \pm 0.15}$
        
         
         \\
        &
         3 & 
        Symbolic&
        Cora & $5.38 {\scriptstyle \pm 0.00}$
        
         
         \\
        &
         3 & 
        Dense&
        CiteSeer &$ 8.42 {\scriptstyle \pm 0.69}$
        
         
         \\
          &
         3 & 
        Symbolic&
        CiteSeer & $5.51 {\scriptstyle \pm 0.04}$
        
         
         \\
         
         
         
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:runtime}
\end{table*}

==> tables/runtime2.tex <==
\begin{table*}[htbp!]
    \centering
    \caption{Results for runtime speedup quantification using symbolic as compared to dense matrices. These results are for the GCN-dDGM-EHS model using $k=3$ and training for 100 epochs using NVIDIA P100 GPU.
    }
    
\scalebox{0.65}{
    \begin{tabular}{ccclc}
    \toprule 
         Model &
         No. dDGMs &
         Matrix &
         Dataset &
         Runtime (s) $\pm$ Standard Deviation
         \\ \midrule

         \multirow{12}{*}{GCN-dDGM-EHS} &
         1 & 
        Dense &
        Cora &  $ 6.17 {\scriptstyle \pm 0.41}$
         \\
          &
         1 & 
        Symbolic&
        Cora &  $ 4.27 {\scriptstyle \pm 0.06 }$
        
         
         \\
        &
         1 & 
        Dense&
        CiteSeer &  $ 7.92 {\scriptstyle \pm 0.33 }$
        
         
         \\
      &
         1 & 
        Symbolic&
        CiteSeer &   $4.38 {\scriptstyle \pm 0.02 }$
        
         
         \\
         &
         2 & 
        Dense&
        Cora &  $10.67 {\scriptstyle \pm 0.32}$
        
         
         \\
          &
         2 & 
        Symbolic&
        Cora & $ 7.18 {\scriptstyle \pm 0.03 }$
        
         
         \\
       &
         2 & 
        Dense&
        CiteSeer &  $ 14.15 {\scriptstyle \pm 0.07}$
        
         
         \\
        &
         2 & 
        Symbolic&
        CiteSeer &  $ 7.48{\scriptstyle \pm 0.16}$
        
         
         \\
         &
         3 & 
        Dense&
        Cora &  $15.32 {\scriptstyle \pm 0.13}$
        
         
         \\
          &
         3 & 
        Symbolic&
        Cora & $ 10.08 {\scriptstyle \pm 0.06}$
        
         
         \\
         &
         3 & 
        Dense&
        CiteSeer &  $ 20.85 {\scriptstyle \pm 0.42}$
        
         
         \\
          &
         3 & 
        Symbolic&
        CiteSeer &  $ 10.31 {\scriptstyle \pm 0.04}$
        \\
         
         
         
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:runtime2}
\end{table*}

==> tables/runtime_k.tex <==
\begin{table*}[ht!]
    \centering
    \caption{Results for runtime speedup quantification using symbolic as compared to dense matrices for different $k=1-30$. These results are for the GCN-dDGM-E model and training for 100 epochs using a Tesla T4 GPU.
    }
    
\scalebox{0.45}{
    \begin{tabular}{cclc}
    \toprule 

        \multicolumn{4}{c}{GCN-dDGM-E} \\
    \midrule
        
         $k$ &
         Matrix &
         Dataset &
         Runtime (s) $\pm$ Standard Deviation
         \\ \midrule
 1 & 
        Dense&
        Cora & $ 4.22 {\scriptstyle\pm 0.14 }$
        
         
         \\
 
         1 & 
        Symbolic&
        Cora & $ 2.84 {\scriptstyle\pm 0.02 }$
        
         
         \\
       
         1 & 
        Dense&
        CiteSeer & $ 5.26 {\scriptstyle \pm 0.06}$
        
         
         \\
      
         1 & 
        Symbolic&
        CiteSeer &  $2.95 {\scriptstyle\pm 0.02}$
        
         
         \\ \midrule
      
         2 & 
        Dense&
        Cora & $4.23 {\scriptstyle \pm 0.06}$
        
         
         \\
     
         2 & 
        Symbolic&
        Cora & $  2.99 {\scriptstyle\pm 0.18 }$
        
         
         \\
     
         2 & 
        Dense&
        CiteSeer & $ 5.29 {\scriptstyle\pm 0.03}$
        
         
         \\
         
         2 & 
        Symbolic&
        CiteSeer & $ 2.98 {\scriptstyle\pm 0.01 }$
        
         
         \\ \midrule
     
         3 & 
        Dense&
        Cora & $ 4.24 {\scriptstyle \pm 0.06}$
        
         
         \\
    
         3 & 
        Symbolic&
        Cora & $ 2.94 {\scriptstyle \pm 0.02 }$
        
         
         \\
       
         3 & 
        Dense&
        CiteSeer &$  5.54 {\scriptstyle \pm 0.24}$
        
         
         \\
     
         3 & 
        Symbolic&
        CiteSeer & $ 3.04 {\scriptstyle \pm 0.03}$
        
         
         \\ \midrule


   
         5 & 
        Dense&
        Cora & $ 4.25 {\scriptstyle \pm 0.11}$
        
         
         \\
   
         5 & 
        Symbolic&
        Cora & $ 2.93 {\scriptstyle \pm 0.01}$
        
         
         \\
  
         5 & 
        Dense&
        CiteSeer &$ 5.41 {\scriptstyle \pm 0.17}$
        
         
         \\
   
         5 & 
        Symbolic&
        CiteSeer & $ 3.02{\scriptstyle \pm 0.11}$
        
         
         \\ 
         
         \midrule
     
         7 & 
        Dense&
        Cora & $ 4.27 {\scriptstyle \pm 0.02}$
        
         
         \\
   
         7 & 
        Symbolic&
        Cora & $ 2.94 {\scriptstyle \pm 0.03 }$
        
         
         \\
     
         7 & 
        Dense&
        CiteSeer &$ 5.44 {\scriptstyle \pm 0.16}$
        
         
         \\
   
         7 & 
        Symbolic&
        CiteSeer & $ 3.11 {\scriptstyle \pm 0.18}$
        
         
         \\ \midrule

     
         10 & 
        Dense&
        Cora & $ 4.30 {\scriptstyle \pm 0.14 }$
        
         
         \\
    
         10 & 
        Symbolic&
        Cora & $ 2.94 {\scriptstyle \pm 0.04}$
        
         
         \\
   
         10 & 
        Dense&
        CiteSeer &$ 5.48 {\scriptstyle \pm 0.21 }$
        
         
         \\
   
         10 & 
        Symbolic&
        CiteSeer & $ 3.01 {\scriptstyle \pm 0.03}$
        
         
         \\ \midrule

         20 & 
        Dense&
        Cora & $ 4.67 {\scriptstyle \pm 0.52}$
        
         
         \\
   
         20 & 
        Symbolic&
        Cora & $ 3.19 {\scriptstyle \pm 0.05 }$
        
         
         \\
 
         20 & 
        Dense&
        CiteSeer &$ 5.49 {\scriptstyle \pm 0.03}$
        
         
         \\
    
         20 & 
        Symbolic&
        CiteSeer & $ 3.14 {\scriptstyle \pm 0.05}$
        
         
         \\ \midrule

         30 & 
        Dense&
        Cora & $ 4.23 {\scriptstyle \pm 0.01 }$
        
         
         \\
     
         30 & 
        Symbolic&
        Cora & $ 3.21 {\scriptstyle \pm 0.20}$
        
         
         \\
   
         30 & 
        Dense&
        CiteSeer &$ 5.25 {\scriptstyle \pm 0.03 }$
        
         
         \\
    
         30 & 
        Symbolic&
        CiteSeer & $ 3.35 {\scriptstyle \pm 0.03 }$
        
         
         \\
         
         
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:runtime_k}
\end{table*}

==> tables/runtime_k2.tex <==
\begin{table*}[ht!]
    \centering
    \caption{Results for runtime speedup quantification using symbolic as compared to dense matrices for different $k=1-30$. These results are for the GCN-dDGM-EHS model and training for 100 epochs using a Tesla T4 GPU.
    }
    
\scalebox{0.45}{
    \begin{tabular}{cclc}
    \toprule 

        \multicolumn{4}{c}{GCN-dDGM-EHS} \\
    \midrule
        
         $k$ &
         Matrix &
         Dataset &
         Runtime (s) $\pm$ Standard Deviation
         \\ \midrule
 1 & 
        Dense&
        Cora & $ 5.46 {\scriptstyle\pm 0.02}$
        
         
         \\
 
         1 & 
        Symbolic&
        Cora & $ 4.50 {\scriptstyle\pm 0.02}$
        
         
         \\
       
         1 & 
        Dense&
        CiteSeer & $ 7.27{\scriptstyle \pm 0.80}$
        
         
         \\
      
         1 & 
        Symbolic&
        CiteSeer &  $ 4.97 {\scriptstyle\pm 0.56 }$
        
         
         \\ \midrule
      
         2 & 
        Dense&
        Cora & $ 5.37{\scriptstyle \pm 0.03 }$
        
         
         \\
     
         2 & 
        Symbolic&
        Cora & $ 4.56 {\scriptstyle\pm 0.02 }$
        
         
         \\
     
         2 & 
        Dense&
        CiteSeer & $ 6.69 {\scriptstyle\pm 0.02 }$
        
         
         \\
         
         2 & 
        Symbolic&
        CiteSeer & $ 4.71 {\scriptstyle\pm 0.03}$
        
         
         \\ \midrule
     
         3 & 
        Dense&
        Cora & $ 5.36 {\scriptstyle \pm 0.02 }$
        
         
         \\
    
         3 & 
        Symbolic&
        Cora & $  4.57 {\scriptstyle \pm 0.16 }$
        
         
         \\
       
         3 & 
        Dense&
        CiteSeer &$ 6.77 {\scriptstyle \pm 0.06}$
        
         
         \\
     
         3 & 
        Symbolic&
        CiteSeer & $ 5.06 {\scriptstyle \pm 0.73}$
        
         
         \\ \midrule


   
         5 & 
        Dense&
        Cora & $ 5.57 {\scriptstyle \pm 0.22}$
        
         
         \\
   
         5 & 
        Symbolic&
        Cora & $ 4.58 {\scriptstyle \pm 0.07 }$
        
         
         \\
  
         5 & 
        Dense&
        CiteSeer &$ 6.74 {\scriptstyle \pm 0.02 }$
        
         
         \\
   
         5 & 
        Symbolic&
        CiteSeer & $ 4.70 {\scriptstyle \pm 0.03 }$
        
         
         \\
         \midrule
     
         7 & 
        Dense&
        Cora & $ 5.62 {\scriptstyle \pm 0.29 }$
        
         
         \\
   
         7 & 
        Symbolic&
        Cora & $ 4.47 {\scriptstyle \pm 0.01 }$
        
         
         \\
     
         7 & 
        Dense&
        CiteSeer &$  6.75 {\scriptstyle \pm 0.05}$
        
         
         \\
   
         7 & 
        Symbolic&
        CiteSeer & $ 4.99 {\scriptstyle \pm 0.58 }$
        
         
         \\ \midrule

     
         10 & 
        Dense&
        Cora & $ 5.92 {\scriptstyle \pm 0.73}$
        
         
         \\
    
         10 & 
        Symbolic&
        Cora & $ 4.70 {\scriptstyle \pm 0.04 }$
        
         
         \\
   
         10 & 
        Dense&
        CiteSeer &$ 7.06 {\scriptstyle \pm 0.43}$
        
         
         \\
   
         10 & 
        Symbolic&
        CiteSeer & $ 4.83 {\scriptstyle \pm 0.03}$
        
         
         \\ \midrule

         20 & 
        Dense&
        Cora & $ 5.44 {\scriptstyle \pm 0.02 }$
        
         
         \\
   
         20 & 
        Symbolic&
        Cora & $ 4.77 {\scriptstyle \pm 0.13 }$
        
         
         \\
 
         20 & 
        Dense&
        CiteSeer &$ 6.76 {\scriptstyle \pm 0.03 }$
        
         
         \\
    
         20 & 
        Symbolic&
        CiteSeer & $ 4.86 {\scriptstyle \pm 0.18}$
        
         
         \\ \midrule

         30 & 
        Dense&
        Cora & $ 5.63 {\scriptstyle \pm 0.30 }$
        
         
         \\
     
         30 & 
        Symbolic&
        Cora & $ 4.74 {\scriptstyle \pm 0.03}$
        
         
         \\
   
         30 & 
        Dense&
        CiteSeer &$ 6.93 {\scriptstyle \pm 0.22}$
        
         
         \\
    
         30 & 
        Symbolic&
        CiteSeer & $5.33 {\scriptstyle \pm 0.66}$
        
         
         \\
         
         
         \bottomrule

         
    \end{tabular}}
    
    \label{tab:runtime_k2}
\end{table*}

==> tables/summary_brain_imaging.tex <==


\begin{table*}[htbp!]
    \centering
    \caption{Summary of model architectures for TadPole.
    }
    
\scalebox{0.83}{
    \begin{tabular}{lc cccc}
    \toprule 
&  & & \multicolumn{3}{c}{Model}
    \\ \midrule
          &
& &
         \textbf{MLP} &  
         \textbf{GCN-dDGM}
         &  
         \textbf{GAT-dDGM}
         \\ \midrule

         
         
         No. Layer parameters & BatchNorm & Activation & \multicolumn{3}{c}{Layer type}
         \\\midrule
          & & & N/A  & dDGM & dDGM
          \\\hdashline
         (No. features, 32) & No & ELU & Linear & Graph Conv & Graph Attention
          \\ 
          (32, 16) & No & ELU & Linear  & Graph Conv & Graph Attention
          \\
          (16, 8) & No & ELU & Linear  & Graph Conv & Graph Attention
          \\ 
          (8, 8) & Yes & ELU & Linear & Linear & Linear
          \\ 
          (8, 8) & Yes & ELU & Linear  & Linear & Linear
          \\ 
          (8, No. classes) & No & -  &  Linear & Linear & Linear
          \\ 
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:Summary of model architecture brain}
\end{table*}

==> tables/summary_of_models_1.tex <==


\begin{table*}[htbp!]
    \centering
    \caption{Summary of model architectures for experiments using classical graph datasets. Most experiments only use the first dDGM module.
    }
    
\scalebox{0.7}{
    \begin{tabular}{lc ccc}
    \toprule 
&  & \multicolumn{3}{c}{Model}
    \\ \midrule
          &
&
         \textbf{MLP} &  
         \textbf{GCN} & 
         \textbf{GCN-dDGM}
         \\ \midrule

         
         
         No. Layer parameters & Activation & \multicolumn{3}{c}{Layer type}
         \\\midrule
          &  & N/A & N/A & dDGM
          \\\hdashline
         (No. features, 32) & ELU & Linear & Graph Conv & Graph Conv
          \\ \hdashline
          &  & N/A & N/A & dDGM
          \\\hdashline
          (32, 16) & ELU & Linear & Graph Conv & Graph Conv
          \\\hdashline
          &  & N/A & N/A & dDGM 
          \\\hdashline
          (16, 8) & ELU & Linear & Graph Conv & Graph Conv
          \\ 
          (8, 8) & ELU & Linear &  Linear & Linear
          \\ 
          (8, 8) & ELU & Linear &  Linear & Linear
          \\ 
          (8, No. classes) & - & Linear &  Linear & Linear
          \\ 
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:Summary of model architecture}
\end{table*}

==> tables/summary_of_models_2.tex <==


\begin{table*}[htbp!]
    \centering
    \caption{Summary of model architectures for experiments using heterophilic graph datasets. The dDGM module uses different $k$ values.
    }
    
\scalebox{0.83}{
    \begin{tabular}{lcc ccc}
    \toprule 
&  & &\multicolumn{3}{c}{Model}
    \\ \midrule
          &
& &
         \textbf{MLP} &  
         \textbf{GCN} & 
         \textbf{GCN-dDGM}
         \\ \midrule

         
         
         No. Layer parameters & BatchNorm & Activation & \multicolumn{3}{c}{Layer type}
         \\\midrule
          &  & & N/A & N/A & dDGM
          \\\hdashline
         (No. features, 16) & No & ELU & Linear & Graph Conv & Graph Conv
          \\
          (16, 8) & No & ELU & Linear & Graph Conv & Graph Conv
          \\ 
          (8, 8) & Yes & ELU & Linear &  Linear & Linear
          \\ 
          (8, No. classes) & No & - & Linear &  Linear & Linear
          \\ 
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:Summary of model architecture 2}
\end{table*}

==> tables/summary_ogbn_arxiv.tex <==


\begin{table*}[htbp!]
    \centering
    \caption{Summary of model architectures for experiments for the OGB-Arxiv dataset using GATv2 diffusion layers. As specified in the table, $k=20$ is used for all experiments.
    }
    
\scalebox{0.78}{
    \begin{tabular}{lcc ccc}
    \toprule 
&  & &\multicolumn{3}{c}{Model}
    \\ \midrule
          &
& &
         \textbf{MLP} &  
         \textbf{GATv2} & 
         \textbf{GATv2-dDGM}
         \\ \midrule

         
         
         No. Layer parameters & BatchNorm & Activation & \multicolumn{3}{c}{Layer type}
         \\\midrule
          &  & & N/A & N/A & dDGM ($k=20$)
          \\\hdashline
         ($\textrm{No. features} = 128$, 40) & No & SiLU & Linear & Graph Attention v2 & Graph Attention v2
          \\
          (40, 40) & No & SiLU & Linear & Graph Attention v2 & Graph Attention v2
          \\
          (40, 40) & No & SiLU & Linear & Graph Attention v2 & Graph Attention v2
          \\

          (40, 40) & Yes & SiLU & Linear &  Linear & Linear
          \\ 
          (40, 100) & Yes & SiLU & Linear &  Linear & Linear
          \\ 
          (100, $\textrm{No. classes} = 40$) & No & - & Linear &  Linear & Linear
          \\ 
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:Summary of model architecture arxiv}
\end{table*}
